LinCQA: Faster Consistent Query Answering with Linear Time Guarantees

Most data analytical pipelines often encounter the problem of querying inconsistent data that violate pre-determined integrity constraints. Data cleaning is an extensively studied paradigm that singles out a consistent repair of the inconsistent data. Consistent query answering (CQA) is an alternative approach to data cleaning that asks for all tuples guaranteed to be returned by a given query on all (in most cases, exponentially many) repairs of the inconsistent data. This paper identifies a class of acyclic select-project-join (SPJ) queries for which CQA can be solved via SQL rewriting with a linear time guarantee. Our rewriting method can be viewed as a generalization of Yannakakis's algorithm for acyclic joins to the inconsistent setting. We present LinCQA, a system that can output rewritings in both SQL and non-recursive Datalog rules for every query in this class. We show that LinCQA often outperforms the existing CQA systems on both synthetic and real-world workloads, and in some cases, by orders of magnitude.

==> fixbuild.tex <==
\makeatletter
\def\set@curr@file#1{%
  \begingroup
    \escapechar\m@ne
    \xdef\@curr@file{\expandafter\string\csname #1\endcsname}%
  \endgroup
}
\def\quote@name#1{"\quote@@name#1\@gobble""}
\def\quote@@name#1"{#1\quote@@name}
\def\unquote@name#1{\quote@@name#1\@gobble"}
\makeatother



==> old-prelim.tex <==
\section{Preliminaries (OLD)}
\label{sec:prelim}

\xiating{Should this section be shorted so that it is more ``SIGMOD'' and less theoretical?}

In this section, we define the notations used in our paper. We assume disjoint sets of {\em variables\/} and {\em constants\/}. We will use $x,y,z, \dots$ to denote variables, and $a,b,c,\dots$ for constants.
% If $\vec{x}$ is a sequence containing variables and constants, then $\var{\vec{x}}$ denotes the set of variables that occur in $\vec{x}$.
% A {\em valuation\/} over a set $U$ of variables is a total mapping $\theta$ from $U$ to the set of~constants.
%At several places, it is implicitly understood that such a valuation $\theta$ is extended to be the identity on constants and on variables not in $U$.
%If $V \subseteq U$, then $\theta[V]$ denotes the restriction of $\theta$ to $V$.

%If $\theta$ is a valuation over a set $U$ of variables, $x$ is a variable, and $a$ is a constant,
%then $\substitute{\theta}{x}{a}$ is the valuation over $U\cup\{x\}$ such that
%$\substitute{\theta}{x}{a}(x)=a$ and for every variable $y$ such that $y\neq x$, $\substitute{\theta}{x}{a}(y)=\theta(y)$.
%Notice that $x\in U$ is allowed.

\introparagraph{Atoms and key-equal facts.}
Let $\vec{x}$ be a sequence containing variables and constants. We denote $\var{\vec{x}}$ as the set of variables that appear in $\vec{x}$. Let $R$ be the relation name, then $R(\underline{\vec{x}}, \vec{y})$ is an atom, where the primary key $\vec{x}$ of $R$ is underlined and we denote $\key{R} = \vec{x}$. 
An {\em $R$-fact\/} (or simply fact or tuple) is an $R$-atom in which no variable occurs.
% Two tuples $R_{1}(\underline{\vec{a}_{1}},\vec{b}_{1}),R_{2}(\underline{\vec{a}_{2}},\vec{b}_{2})$ are said to be {\em key-equal\/} if $R_{1}=R_{2}$ and $\vec{a}_{1}=\vec{a}_{2}$.
%An $R$-atom or an $R$-fact is {\em simple-key\/} if $R$ is simple-key.


% We consider only $2$-ary \emph{relation names}, where the first position is called the \emph{primary key}.
% If $R$ is a relation name, and $s,t$ are variables or constants,
% then $R(\underline{s},t)$ is an \emph{atom}.
% An atom without variables is a \emph{fact}.
% Two facts are \emph{key-equal} if they use the same relation name and agree on the primary key.
%Each {\em relation name\/} $R$ of arity $n$, $n\geq 1$, has a unique {\em primary key\/} which is a set $\{1,2,\dots,k\}$ where $1\leq k\leq n$.
%We say that $R$ has {\em signature\/} $\signature{n}{k}$ if $R$ has arity $n$ and primary key $\{1,2,\dots,k\}$. 
%We say that $R$ is {\em simple-key\/} if $k=1$.
%Elements of the primary key are called {\em primary-key positions\/},
%while $k+1$, $k+2$, \dots, $n$ are {\em non-primary-key positions\/}. 
%For all positive integers $n,k$ such that $1\leq k\leq n$, we assume denumerably many relation names with signature $\signature{n}{k}$.
%Every {\em relation name\/} $R$ has a fixed {\em signature\/}, which is a pair $\signature{n}{k}$ with $n\geq k\geq 1$: the integer $n$ is the {\em arity\/} of the relation name and $\{1,2,\dots,k\}$ is the {\em primary key\/}. 
%
%If $R$ is a relation name with signature $\signature{n}{k}$, then $R(s_{1},\dots,s_{n})$ is called an {\em $R$-atom\/} (or simply atom), where each $s_{i}$ is either a constant or a variable ($1\leq i\leq n$).
%Such an atom is commonly written as $R(\underline{\vec{x}},\vec{y})$ where the primary key value $\vec{x}=s_{1},\dots,s_{k}$ is underlined and $\vec{y}=s_{k+1},\dots,s_{n}$.

%We will use letters $F,G,H$ for atoms.
%For an atom $F=R(\underline{\vec{x}},\vec{y})$, we denote by $\keyvars{F}$ the set of variables that occur in $\vec{x}$,
%and by $\atomvars{F}$ the set of variables that occur in $F$, that is, $\keyvars{F}=\sequencevars{\vec{x}}$ and $\atomvars{F}=\sequencevars{\vec{x}}\cup\sequencevars{\vec{y}}$.

\introparagraph{Database instances, blocks, and repairs.}
A {\em database schema\/} is a finite set of relation names.
All constructs that follow are defined relative to a fixed database schema.

A {\em database instance\/}  $\db$ is a finite set of tuples using only the relation names of the schema.
%We refer to databases as ``uncertain databases'' to stress that such databases can violate primary key constraints.
%
% We denote $\adom{\db}$ as the active domain of $\db$ (i.e., the set of constants that occur in $\db$).
A {\em block\/} of $\db$ is a maximal set of tuples of $\db$ with the same key.
%The term $R$-block refers to a block of $R$-facts, i.e., facts with relation name $R$.
Whenever a database instance $\db$ is understood, we denote $R(\underline{\vec{c}},*)$ as the block containing all tuples with primary-key value~$\vec{c}$ in relation $R$.
%If $A$ is a fact of $\db$, then $\theblock{A}{\db}$ denotes the block of $\db$ that contains $A$.
A database instance $\db$ is {\em consistent\/} if it does not contain distinct tuples that are key-equal (i.e., if no block of $\db$ contains more than one tuple). A {\em repair\/} of $\db$ is an inclusion-maximal consistent subset of $\db$. 
%
%We write $\repairs{\db}$ for the set of repairs of $\db$.


\introparagraph{Conjunctive Queries.}
%A {\em Boolean query\/} is a mapping $q$ that associates a Boolean (true or false) to each uncertain database, such that $q$ is closed under isomorphism.
%We write $\db\models q$ to denote that $q$ associates true to $\db$, in which case $\db$ is said to {\em satisfy\/} $q$.
%A {\em Boolean first-order query\/} is a Boolean query that can be defined in first-order logic (with equality and constants, but without other built-in predicates).
We define a \emph{Conjunctive Query (CQ)} $q$ as a rule of the following form:
%
\begin{align}\label{eq:rule}
q(\vec{u}) \obtainedfrom R_{1}(\underline{\vec{{x}_{1}}},\vec{{y}_{1}}), \dots, R_{n}(\underline{\vec{{x}_{n}}},\vec{{y}_{n}})
\end{align}
%
where each $R_{i}(\underline{\vec{{x}_{i}}},\vec{{y}_{i}})$ is an atom for $1 \leq i \leq n$. We denote by $\queryvars{q}$ the set of variables that occur in $q$ and $\vec{u}$ is said to be the \emph{free variables} of $q$. The atom $q(\vec{u})$ is the \emph{head} of the rule, and the remaining atoms are called the \emph{body} of the rule. 


%The query $q$ represents the first-order sentence with free variables $\vec{u}$: $\exists u_{1}\dotsm\exists u_{k}\normalformula{R_{1}(\underline{\vec{x_1}}, \vec{y_1})\land\dotsm\land R_{n}(\underline{\vec{{x}_{n}}},\vec{{y}_{n}})}$, where $\{u_{1}, \dots, u_{k}\} \cup \var{\vec{u}}=\queryvars{q}$. 
A CQ $q$ is Boolean (BCQ) if it has no free variables, and it is {\em full} if all its variables are free.
We say that $q$ has a {\em self-join\/} if some relation name occurs more than once in $q$.
A CQ without self-joins is called {\em self-join-free\/}. A CQ $q$ is \emph{connected} if there are no two CQs $q_1, q_2$ such that $q = q_1 \cup q_2$ and $\var{q_1} \cap \var{q_2} = \emptyset$. 


For a CQ $q$, let $\vec{x} = \langle x_1, \dots , x_{\ell} \rangle$ be a sequence of distinct variables that occur in $q$ and
$\vec{a} = \langle a_1, \dots , a_{\ell}\rangle$ be a sequence of constants, then $q_{[\vec{x} \rightarrow \vec{a}]}$ denotes the query obtained from $q$ by replacing all occurrences of $x_i$ with $a_i$ for all $1 \leq i \leq \ell$.


%If $q$ has no self-join, then it is called {\em self-join-free\/}.
%By a little abuse of notation, we may confuse atoms with their relation names in a self-join-free Boolean conjunctive query $q$.
%That is, if we use a relation name $R$ at places where an atom is expected,
%then we mean the (unique) $R$-atom of~$q$.

%If $q$ is a Boolean conjunctive query, $\vec{x}=\tuple{x_{1},\dots,x_{\ell}}$ is a sequence of distinct variables that occur in $q$, and $\vec{a}=\tuple{a_{1},\dots,a_{\ell}}$ is a sequence of constants,
%then $\substitute{q}{\vec{x}}{\vec{a}}$ denotes the query obtained from $q$ by replacing all occurrences of $x_{i}$ with $a_{i}$, for all $1\leq i\leq\ell$.

\introparagraph{Datalog.} A Datalog program $P$ is a finite set of rules of the form~\eqref{eq:rule},
with the extension that negated atoms can be used in rule bodies. A rule can be interpreted as a logical implication: if the body is true, then so is the head of the rule. We assume that rules are always safe: this means that every variable that occurs in the rule, must also occur in a non-negated atom of the rule body.
A relation is an IDB relation if it is used in the head of some rule; otherwise it is an EDB relation (i.e., input relation).

Our rewriting uses non-recursive Datalog with negation. This means that the rules of a Datalog program $P$ can be partitioned into $(P_{1},P_{2},\dots,P_{n})$ such that the rule body of a rule in $P_{i}$ uses only IDB predicates defined by rules in some $P_{j}$ with $j<i$.
Here, it is understood that all rules with the same head predicate belong in the same partition.  

%The expressions $h$, $p_1$,$\dots$,$p_k$ are \emph{atoms}, i.e., formulas of the form $R(t_1, \dots , t_{\ell})$, where $R$ is a table/relation name (predicate) and each $t_i$ is a \emph{term} that can be either a constant or a variable. An atom is a \emph{fact} (or \emph{tuple}) if all $t_i$'s are constants.
%The atom $h$ is the \emph{head} of the rule, and the set of atoms $p_1$, $\dots$, $p_k$ is called the \emph{body} of the rule. 


\introparagraph{Consistent query answering.}
For every CQ $q$, given an input database instance $\db$, the problem $\cqa{q}$ asks for the intersection of all query outputs $q(\rep)$ for all repair $\rep$ of $\db$. If $q$ is Boolean, the problem $\cqa{q}$ then asks whether $q$ is satisfied by every repair of the input database instance~$\db$. 

The problem $\cqa{q}$ has a first-order rewriting (\FO-rewriting) if there is another CQ $q'$ such that evaluating $q'$ on the input database $\db$ would return the answers of $\cqa{q}$.	

% It is straightforward that for every BCQ $q$, $\cqa{q}$ is in \coNP.

% \introparagraph{Attack graph.} Let $q$ be a self-join-free BCQ. We define $\FD{q}$ as the following set of functional dependencies:
% $$\FD{q} := \{\fd{\key{F}}{\var{F}} \mid F \in q\}.$$
% %
% For every atom $F \in q$, we define $\keyclosure{F}{q}$ as follows:
% $$\keyclosure{F}{q} := \{x \in \var{q} \mid \FD{q \setminus \{F\}} \models \fd{\key{F}}{x}\}.$$

% The attack graph of $q$ is a directed graph whose vertices are the atoms of $q$. There is a directed edge from $F$ to $G$ $(F \neq G)$ if there exists a sequence $F_0, F_1, \dots, F_n$ of (not necessarily distinct) atoms of $q$ such that
% \begin{itemize}
% 	\item $F_0 = F$ and $F_n = G$; and
% 	\item for all $i \in \{0, \dots , n-1\}$, $\var{F_i} \cap \var{F_{i+1}} \nsubseteq \keyclosure{F}{q}$.
% \end{itemize}
% %\jef{An equivalent, but somewhat more insightful definition is:
% %if there exists a non-empty sequence of variables
% %$$x_{1},x_{2},\ldots,x_{n}$$ 
% %such that no $x_{i}$ is in $\keyclosure{F}{q}$, the leftmost variable occurs in~$F$, the rightmost variable occurs in~$G$, and every two adjacent variables occur together in some atom of~$q$. }
% A directed edge from $F$ to $G$ in the attack graph of $q$ is also called an attack from $F$ to $G$, denoted by $F \attacks{q}G$. 
The attack graph of $q$ is used to determine the data complexity of $\cqa{q}$.

\begin{theorem}[\cite{KoutrisW17}] \label{thm:fo}
Let $q$ be a self-join-free BCQ. Then the attack graph of $q$ is acyclic if and only if $\cqa{q}$ is in \FO.
\end{theorem}

\xiating{Add examples here perhaps? The attack graph of $q = R(\underline{x}, y), S(\underline{y}, x)$ is cyclic but the attack graph of $q' = R(\underline{x}, y), S(\underline{y}, x), T(\underline{y}, x)$ is acyclic.}


==> review.tex <==
\onecolumn
\section*{VLDB Reviews}
\label{sec:response}

\xiating{Common reviews:

\begin{enumerate}
\item Experiments on real world data, or more ``appropriate'' database generator;
\item Motivation for CQA;
\item How much does PPJT extend beyond $\cforest$, because class-wise seems just some key-key join queries, and performance-wise comparable to ConQuer;
\item Intuition for the rewriting rules.
\end{enumerate}

Todo List:
\begin{enumerate}
	\item implement \system
	\item use the semantic definition of ``being reifiable'' and skip introducing attack graphs
	\item real world data
	\item emphasize (a) linear time guarantee (b) wider class than $\cforest$ and (c) as fast as ConQuer (and sometimes faster)
\end{enumerate}
}
% \begin{enumerate}
% 	\itemsep0em
% 	\item \ansm{Common changes for multiple reviewers and updates in the presentation of the paper are in RED.}
% 	\item \ansa{Reviewer 1 in PURPLE.}
% 	\item \ansb{Reviewer 2 in BROWN.}
% 	\item \ansc{Reviewer 3 in MAGENTA.}
% \end{enumerate}


\subsection*{Meta-review}
	\ques{The main concerns of the reviewers were about the motivation of the problem and the clarification of the correctness of the approach which need major improvement.

We hope that the detailed reviewers' comments can help the authors to improve the current version of the paper for a next iteration and submission, and also offer interesting research directions.} \\
	

\subsection*{Reviewer 1}
\begin{enumerate}
	\item(R1-W1) \ques{Presentation can be improved, with plenty of minor errors and description of the proposed approaches which is not easy to understand.}
	
	\item(R1-W2) \ques{The paper contains several symbols and the examples, lemmas are hard to understand.} 
	\item(R1-W3) \ques{Intuitions of the Rewriting rules are not clear.}
	\xiating{To be addressed.}
	\item(R1-W4) \ques{The experimental section can be organized better, and the related discussions on the results should be improved.}
	\xiating{To be addressed.}
	\item(R1-D1) \ques{The presentation should be improved. It is hard to follow the intuitions of the sub-sections. Some of the examples (e.g., Example 4.1) are not clear. This particular section needs improvement in the presentation.} 
	\xiating{To be addressed.}
	\item(R1-D2) \ques{The discussions on the experimental findings should be highlighted systematically using the query properties.}
	\xiating{Unclear to me.}
	\item(R1-D3) \ques{The rules are not clear in Section 4.2. The intuitions of the rules should be written properly (e.g., Rule 3).}
	
	\item(R1-D4) \ques{In experimental section: list the parameters used in the experiments and then vary them within the range to demonstrate the findings}

\end{enumerate}

\subsection*{Review 2}
\begin{enumerate}
	\item(R2-W1) \ques{The motivation needs to be more clearly positioned.}
	
	\item(R2-W2) \ques{My main concern is the readability of the paper. It is quite difficult to be understood with many important concepts unclearly explained.}
	
	\item(R2-W3) \ques{The experiments need to be improved.}
	

	\item(R2-D1) \ques{The motivation example seems to be made on purpose. Besides, in this example, it seems that performing data cleaning (e.g., with the help of crowdsourcing) before consistent query answering is more preferable.} 
	\xiating{To be addressed.}

	\item(R2-D2) \ques{The paper is quite difficult to be understood with many important concepts unclearly explained.
For example, what are the repairs of the inconsistent database?
What is the exact meaning of FO-writable queries?
Although the concept“attack graph”was proposed in another paper (the authors do not put the citation properly when it is first used in this paper), it is not clearly discussed. As the concept is quite important for PPJT, examples for the attack graph are of great necessity.
It would be much more helpful to readers if the authors elaborate concepts, data structures, and methods in Section 4 and Section 5 using a consistent example.}
	
	\item(R2-D3) \ques{Will the order of atoms matter in PPJT? How to decide the order of atoms of the BCQ.}
	
	\item(R2-D4) \ques{In my opinion, the consistent query answering can be modeled as discovering graph functional dependencies, in which the relational databases are models as graphs. It would be more helpful if the authors can make a careful discussion with the following work.
	\begin{itemize}
\item Wenfei Fan, Chunming Hu, Xueli Liu, and Ping Lu, Discovering Graph Functional Dependencies, ACM Transactions on Database Systems (TODS), 2020
\item Wenfei Fan, and Ping Lu, Dependencies for Graphs ACM Transactions on Database Systems (TODS) 44(2): 5:1-5:40 (invtied), 2019.
\item Wenfei Fan, Chunming Hu, Xueli Liu, and Ping Lu, Discovering Graph Functional Dependencies, ACM SIGMOD Conference on Management of Data (SIGMOD), 2018.
\end{itemize}
}
	
	\item(R2-D5) \ques{ The number of join relations for the synthetic workload is not evaluated.}

\end{enumerate}

\subsection*{Review 3}

\begin{enumerate}
	
	\item (R3-W1) It remains unclear what the practical relevance of the proposed work is. Neither the motivation in the introduction nor the evaluation indicate or validate how the proposed work benefits or potentially performs in realistic real-life applications.
	
	\xiating{To be addressed.}
	
	\item (R3-W2) Quite a few ideas, including the central notions of PPJTs to rewritings and the “main result” of Theorem 4.6. apply / extend / are similar to related work. It remains unclear to me to what extend the work presented are original contributions.

	\xiating{To be addressed in the presentation.}

	\item (R3-W3) The evaluation limits to quite artificial benchmarks that, as far as I can tell, do not reflect realistic scenarios. It is thus difficult to generalize the results to any practical setting.
	
	\xiating{To be addressed with real datasets.}

	\item (R3-D1) As mentioned in W1, I see one opportunity of improvement with respect to the motivation and relevance of the contribution for practical applications. To avoid misunderstanding, I do not expect a fully fledged and deployed real-world use case with real data in the motivation and evaluation. However, I would expect some argument and description in what settings / scenarios the proposed solution is preferable over the widely used approach in practice.

	\xiating{To be researched?}

\item (R3-D2) The original contribution is, at least from my understanding of reading the paper, somewhat limited. The paper extends the work of Yannanakis (on consistent databases) to databases with one specific kind of inconsistency in keys. The class of queries considered only slightly extends the class covered by the paper cited as [28] and it remains unclear how relevant this extension is in practice (cf W1). Indeed, the paper itself mentions that [28] “covers most of the queries seen in practical settings”. Also, the query rewriting algorithm is based on the work cited as [45]. From a theoretical perspective, a contribution as the one mentioned as future work would be more compelling as it would not cover a very special case only. From a practical perspective, from the experiments, it seems any of the existing CQA algorithms based on query rewriting would be fine as they yield results in 1 second or less on all but the largest tpc-h experiments (where rewritten queries require <4 s). How they behave or apply in more realistic settings remains an open question.

	\xiating{To be addressed and discussed.}

\item (R3-D3) In the description of the queries of the synthetic workload, the text mentions they include projection and joins. How about selections? The use of variable d suggests this is a constant. If so, how is it set and how do you guarantee the selectivity has not significant impact on your conclusions?

	\xiating{To be addressed, constants and selection happens at the self-pruning phase.}

\item (R3-D4) The generated data as described in the paragraph “consistent data generation” is far from any realistic data distribution. Also, the addition of inconsistencies seems too homogeneous to reflect real-life situations. In the evaluation, I would appreciate a benchmark that better reflects real-life settings (in addition to studying the effect of varying key parameters in a realistic setting). While I understand finding real-world data (and queries) is difficult, a more general database generator would already be very helpful to further vary the settings covered by the benchmark and thus allowing more general conclusions on how the algorithms behave in different settings.
\xiating{Better databse generator?}

\item (R3-D5) The workloads over both datasets are fixed and it is unclear why this set of queries is well suited, e.g., by covering various workload characteristics. I would appreciate a more systematic variation of the queries (e.g., varying number of joins, number of different join categories such as key-foreign key, key-key, non-key-non key, etc. selectivity, varying projection, selection, etc.). This may allow more better differentiated results with respect to different query categories, for instance. That such effects exist may be the underlying reason for the “gap” in performance changing between TPC-H and synthetic scenarios. Or they lie in the data (cf D4). In any case, this requires further investigation.

\xiating{To be addressed.}

\item (R3-D6) The worst-case study nicely confirms the theoretical results. However, I would suggest adding a discussion on how frequent such cases potentially are. This would allow to better assess whether the work is most beneficial in a very rare corner case only or if its results may have some larger impact. From the TPC-H evaluation, Conquer seems to be most adequate for most practical settings.

\xiating{To be addressed and further argued.}
\end{enumerate}



==> revision.tex <==
% \twocolumn
\section*{Response Letter for Paper 142:  ``LinCQA: Faster Consistent Query Answering with Linear Time Guarantees''}
\label{sec:response}
%We thank the reviewers for the revision opportunity and their clear, constructive reviews. To address the feedback, we have made major changes to the manuscript. Updates made in response to the comments are color-coded as follows. 
We thank the reviewers for their insightful and constructive comments, which we address in this revision. Responses to reviewers' comments and the main changes made to the manuscript are color-coded as follows. 
\begin{enumerate}
	\itemsep0em
	%\item \ansm{Common changes for multiple reviewers and updates in the presentation of the paper are in RED.}
	%\item \ansa{Reviewer \#1 in PURPLE.}
	%\item \ansb{Reviewer \#3 in MAGENTA.}
	%\item \ansc{Reviewer \#4 in BROWN.}
	\item \ansm{Responses \& changes addressing common feedback from multiple reviewers and meta-reviews are in RED}
	\item \ansa{Responses \& changes addressing additional comments from Reviewer \#1 in PURPLE.}
	\item \ansb{Responses \& changes addressing additional comments from Reviewer \#3 in MAGENTA.}
	\item \ansc{Responses \& changes addressing additional comments from Reviewer \#4 in BROWN.}
\end{enumerate}
\noindent
The extended version of this paper is accessible at this link: {\color{blue} \url{https://anonymous.4open.science/r/LinCQA-251E/paper.pdf}}.
%\xiating{change!}

\subsection*{Meta-review}
	\begin{enumerate}
		\item {\bf R1O1, R1O2, R4O1} : Aim for a self-contained paper that depends less on an extended version. %This particularly relates to the core notion of attacks that should at least be introduced in your text. Where still required, make references to the extended version clear and explicit. \\
		%\ansm{We added the definition of attacks to Section~\ref{sec:prelim} and compare our algorithm to Yannakakis' algorithm in Section~\ref{sec:ppjt}. 
		\\
		\ansm{We added the definition of acyclic queries, join trees and attack graphs in Section~\ref{sec:prelim} and compare our algorithm to Yannakakis' algorithm in Section~\ref{sec:ppjt}, which are sufficient preliminaries for understanding our rewriting algorithm.	
		% The intuitions and a correctness argument for our rewriting rules are added to Section~\ref{sec:datalog}. 
		% The formal correctness proof is in Section~\ref{sec:correctness-boolean}. 
		The extended version now contains only complementary results: an efficient construction of PPJT for Section~\ref{sec:ppjt}, our detailed improvements to existing systems for Section~\ref{sec:existing-cqa-systems}, more experimental results for Section~\ref{sec:experiments}, and formal proofs for Proposition~\ref{prop:ppjt},~\ref{prop:cforest}, Lemma~\ref{lemma:parameterization}, Theorem~\ref{thm:main:boolean} and~\ref{thm:main:full}.}
		
		\item {\bf R3O2, R3O5} : Improve readability and organization of the text and aim for economical use of notation. %(Be advised that this is a *major* issue that will be judged critically by the reviewers.) \\
		\\
		\ansm{We have significantly rewritten Section~\ref{sec:rewriting} to improve the readability, adding intuitive examples and using notation only when needed: %The current structure is:
			\begin{itemize}
				%\item In Section~\ref{sec:ppjt}, we introduce the PPJT, its properties and the class of queries it captures;
				\item At the beginning of Section~\ref{sec:rewriting}, we simplified the original example query for easier understanding;  
				\item In Section~\ref{sec:datalog}, we present the intuitions and the detailed rewriting rules for $\cqa{q}$ for any Boolean CQ $q$ with a PPJT using minimal definitions and notations. A more detailed example is added in Figure~\ref{fig:example-rewriting}. We also compare it with Yannakakis' algorithm and argue for its correctness; and
				% We postpone the formal proof of Theorem~\ref{thm:main:boolean} in Appendix~\ref{sec:correctness-boolean} of the extended version; and
				\item In Section~\ref{sec:nonboolean}, we made corresponding changes to extension to non-Boolean CQs. 
				% The formal proof of Theorem~\ref{thm:main:full} is in Appendix~\ref{proof:thm:main:full}
			\end{itemize}
		 } 
		\ansb{We note that since many of the other comments from \textbf{R3} address the readability and organization and complements \textbf{R3O2} and \textbf{R3O5}, most changes made in Section~\ref{sec:rewriting} are highlighted in PURPLE}
		\item {\bf R4O2} : Discuss whether/how LinCQA provides benefits over ConQuer. \\
		%\ansm{We compare the performance of \system\ and ConQuer for each experiment, and provided a summary at the end of Section~\ref{sec:experiments}.}
		\ansm{Compared to ConQuer, we emphasize that LinCQA is applicable to a wider class of acyclic queries, performs obviously better on large datasets despite comparable performance observed on small to medium sized databases (Section~\ref{sec:exp_results}), and  
		  significantly outperforms ConQuer on worst-case instances due to its robustness (Section~\ref{sec:worst}).}
		\item {\bf R3O10, R4O3} : Include a discussion of your observations (including result size, see R3O10) when the source and intermediate tables during query processing exceed the main memory size. \\
		\ansm{Table~\ref{tbl:every-dataset} presents the sizes of consistent and possible answers for selected datasets. %We also compared the performance of all systems on the StackOverflow dataset on various maximum memory allowed and presented the results in Figure~\ref{fig:stackoverflow-memory}.} 
		 We added Figure~\ref{fig:stackoverflow-memory} presenting the results of experiments on SQL server under various amounts of available memory, using the StackOverflow dataset.}
\end{enumerate}
	

\subsection*{Reviewer \#1}
%\begin{enumerate}
%	\item(R1O3) \ques{On the proof of Theorem~\ref{thm:main:full}.} \\
%	\ansa{We introduce the algorithms in the proof sketch of Theorem~\ref{thm:main:full} and postpone the formal correctness proof in Appendix~\ref{proof:thm:main:full}.}
%	\item(R1O4) \ques{On extension to non-acyclic queries.} \\
%	\ansa{We added some discussions on the future works. However, as noted near Proposition~\ref{prop:non-ppjt-linear} of the extended version, an extention to acyclic BCQs without a PPJT is challenging.}
%	\item(R1O5) \ques{On the inconsistencies in the StackOverflow dataset.}
%	\ansa{We added an emphasis on the quasi-keys.}
%\end{enumerate}
Besides what have been covered in the meta-reviews, we addressed additional comments as follows:
\ansa{
    \begin{itemize}
        \item \textbf{R1O3}: We introduced the algorithms in the proof sketch of Theorem~\ref{thm:main:full} in Section~\ref{sec:nonboolean} and postpone the formal correctness proof in Appendix~\ref{proof:thm:main:full}.
        \item \textbf{R1O4}: We added some discussions on future works. However, as noted near Proposition~\ref{prop:non-ppjt-linear} of the extended version, an extension to acyclic BCQs without a PPJT is challenging.
        \item \textbf{R1O5}: We made clarification on primary keys (which are quasi-keys) in Section~\ref{sec:stackoverflow}.
    \end{itemize}
We also addressed points mentioned in minor remarks. 
}

\subsection*{Reviewer \#3}
Besides what have been covered in the meta-reviews, we addressed additional comments as follows:
%\begin{enumerate}
%	\item \textbf{R3O1}: %\ques{On the broadness of the supported class of queries and frequency in realistic workload.
%}\\
%	\ansb{We have added a discussion on the broadness of the supported class of query near Proposition~\ref{prop:cforest}. 
	% In particular, we showed that PPJT captures all \FO-rewritable queries that joins two distinct tables, which are frequent in production.
%	}
%	\item(R3O3) \ques{On data complexity vs.\ combined complexity.}\\
%	\ansb{We added in Section~\ref{sec:prelim} that we study the data complexity of $\cqa{q}$.}
%	\item(R3O4) \ques{On motivation and correctness of the rewriting rules.}\\
%	\ansb{We added intuitions and a correctness argument to our rewriting rules in Section~\ref{sec:datalog}, together with a new running example in Figure~\ref{fig:example-rewriting}. The formal correctness proof is in Appendix~\ref{sec:correctness-boolean}.}
%	\item(R3O8) \ques{What do IDB and EDB stand for?}
%	\ansb{We added the full names in Section~\ref{sec:prelim}.}
%	\item(R3O9) \ques{On using BART for inconsistency injection.}\\
%	\ansb{We provided some references to alternative inconsistency injection options in Section~\ref{sec:experiments}.}
	% \item(R3O6) \ques{ A more general question is whether the proposed types of repairs are actually useful today. That is, the repairs that are returned “delete” records from the query answer, to generate an instance that is violation-free. However, V-repairs are now the norm in integrity constraint data cleaning (cleaning records by value modification and not by tuple deletion). Moreverer, since one could have multiple valid repairs, the authors did not address the often-hard data repairing question of: which repair is (actually) the correct one?}\\
	% \ansb{skip}
	% \item(R3O7) \ques{For non-boolean queries, it is unclear whether the proposed solution would provide a single consistent query answer or would generate a SQL query for each possible consistent repair.}\\
	% \ansb{skip}
	% \item(R3O11) \ques{The experimental study did not address repair quality at all. At the end of the day, data repairing is about making/returning (correct) data. So, correctness of repair is often evaluated in the data cleaning literature. I understand that the authors focused on the problem of query rewriting only, however, I am not sure if this is enough for a SIGMOD paper.}\\
	% \ansb{skip}
%\end{enumerate}
\ansb{
    \begin{itemize}
    	\item \textbf{R3O1}: We added a discussion on the broadness of the supported class of queries near Proposition~\ref{prop:cforest}. 
	\item \textbf{R3O3}: We now have made it clear in Section~\ref{sec:prelim} that we study the data complexity of $\cqa{q}$.
	\item \textbf{R3O4}: We added intuitions and a correctness argument to our rewriting rules in Section~\ref{sec:datalog}, together with a new running example in Figure~\ref{fig:example-rewriting}. The formal correctness proof is in Appendix~\ref{sec:correctness-boolean}. 
	\item \textbf{R3O8}: We added the full names in Section~\ref{sec:prelim}.
	\item \textbf{R3O9}: We noted alternative inconsistency injection options in Section~\ref{sec:experiments}.
    \end{itemize}
}


\subsection*{Reviewer \#4}
\ansc{Major concerns \textbf{R4O1}, \textbf{R4O2}, and \textbf{R4O3} are addressed in meta-reviews. We also changed all figures to be in logarithmic scale with base~$10$.}


==> rewriting_old.tex <==

\section{A Linear-Time Rewriting}\label{sec:rewriting}

Before presenting our linear-time rewriting for $\cqa{q}$, we first provide a motivating example.
Consider the following query on the \database{Company} database shown in Figure~\ref{fig:incon_db_example}:

% \xiating{A more natural example?}
\renewcommand{\quote}{\list{}{\rightmargin=\leftmargin\topsep=0pt}\item\relax}
\vspace{0.5ex}
\begin{quote}
\emph{
% Is there an office whose contact person manages the office since 2020 and, moreover, works from home in the same city as the office?
\revm{
% Is there an employee who works, manages, serves as the contact person of the same office and starts in 2020?
Is there an office whose contact person works for the office and, moreover, manages the office since 2020?
}
}
\end{quote}
\vspace{0.5ex}
% This query can be expressed as the following SQL query: 
%
% \begin{lstlisting}
%           SELECT DISTINCT 1
%           FROM Employee E, Manager M, Contact C
%           WHERE E.employee_id = M.manager_id 
%             AND M.manager_id = C.contact_id
%             AND E.office_city = E.wfh_city 
%             AND E.office_city = M.office_city 
%             AND M.office_city = C.office_city
%             AND M.start_year = 2020 ;
% \end{lstlisting}


% We can also express the query using a non-recursive Datalog rule, where the underlined attributes denote the primary key positions.
\noindent
This query can be expressed by the following CQ:
%
% \begin{align*}
% \examplequery() \obtainedfrom \relation{Employee}(\underline{x}, z, z), \relation{Manager}(\underline{z}, x, \texttt{2020}), \relation{Contact}(\underline{z}, x).
% \end{align*}
\revm{
\begin{align*}
\examplequery() \obtainedfrom \relation{Employee}(\underline{x}, y, z), \relation{Manager}(\underline{y}, x, \texttt{2020}), \relation{Contact}(\underline{y}, x).
\end{align*}
}
To the best of our knowledge, the most efficient running time for $\cqa{\examplequery}$ guaranteed by existing systems  is quadratic in the input database size, denoted~$N$.
The problem $\cqa{\examplequery}$ admits an \FO-rewriting by the classification theorem in \cite{DBLP:conf/pods/KoutrisOW21}.
However, the non-recursive Datalog rewriting of $\cqa{\examplequery}$ produced by Conquesto contains cartesian products between two tables, which means that it runs in $\Omega(N^2)$ time in the worst case. 
Also, since $\examplequery$ is not in $\mathcal{C}_{\mathsf{forest}}$, ConQuer cannot produce an \FO-rewriting. 
% The only attacks are $\relation{Employee}\attacks{}\relation{Manager}$ and $\relation{Employee}\attacks{}\relation{Contact}$, and so the attack graph of $\examplequery$ is acyclic. Thus, by Theorem~\ref{thm:fo}, $\cqa{\examplequery}$ can be solved via an \FO-rewriting. 
Both EQUIP and CAvSAT solve the problem through Integer Programming or SAT solvers, which can take exponential time.
% \jef{Well, they guarantee $O(2^{N})$, which is better than $O(2^{2^{N}})$. Maybe say: ``which can take exponential time.''}
%Hence, the existing systems that rely on Binary Integer Programming or Satisfiability solvers (e.g., EQUIP, CAvSAT) are an overkill and cannot guarantee termination in polynomial time.
One key observation is that $\examplequery$ requires a primary-key to primary-key join and a non-key to non-key join at the same time. As will become apparent in our technical treatment in Section~\ref{sec:datalog}, this property allows us to solve $\cqa{\examplequery}$ in $O(N)$ time, while existing CQA systems will run in more than linear time.

The remainder of this section is organized as follows. In Section~\ref{sec:ppjt}, we introduce the pair-pruning join tree (PPJT). In Section~\ref{sec:datalog}, we consider every Boolean query $q$ having a PPJT and present a novel linear-time non-recursive Datalog program for $\cqa{q}$ (Theorem~\ref{thm:main:boolean}). Finally, we extend our result to all acyclic self-join-free CQs in Section~\ref{sec:nonboolean} (Theorem~\ref{thm:main:full}) . 


\subsection{Pair-pruning Join Tree}
\label{sec:ppjt}

Here we introduce the notion of a {\em pair-pruning join tree} (PPJT). We first assume that the query $q$ is connected, and then discuss how to handle disconnected queries at the end of the section.

Whenever a self-join-free query is understood, we can use a relation name wherever an atom is expected.
For example, we may use $\relation{Employee}$ as a shorthand for the atom $\relation{Employee}(\underline{x},y,z)$ in $\examplequery$.

% The following definition requires a technical notion of an \emph{attack}, a binary relation on the atoms of a self-join-free CQ $q$. \footnote{Details about the attacks and attack graphs can be found in \cite{DBLP:conf/pods/KoutrisOW21}.}
% For the understanding of this paper, it is sufficient to know that informally, if $\cqa{q}$ admits an \FO-rewriting and an atom $R$ attacks an atom $S$ in $q$, then the table $R$ must join with table $S$ from the outside of any \FO-rewriting of $\cqa{q}$. \xiating{needs revision...}


\begin{definition}[PPJT]
\label{defn:ppjt}
Let $q$ be an acyclic self-join-free BCQ. Let $\tau$ be a join tree of $q$ and $R$ a node in $\tau$. The tree $(\tau, R)$ is a \textit{pair-pruning join tree (PPJT)} of $q$ if for any rooted subtree $(\tau', R')$ of $(\tau, R)$, the atom~$R'$ is unattacked in $q_{\tau'}$.
\end{definition}

%\jef{
%Not clear why pair-pruning was chosen as a name. To guide the reader, it might be useful to explain the intuition behind this name.
%}


\begin{example}
For the join tree $\tau$ in Figure~\ref{fig:join-tree},
the rooted tree $(\tau, \relation{Employee})$ is a PPJT for $\examplequery$. The atom $\relation{Employee}(\underline{x}, y, z)$ is unattacked in $q$. For the child subtree $(\tau_M, \relation{Manager})$ of $(\tau, \relation{Employee})$, the atom $\relation{Manager}(\underline{y}, x, \texttt{2020})$ is also unattacked in the following subquery
% 
\begin{align*}
\examplequery_{\tau_M}() \obtainedfrom \relation{Manager}(\underline{y}, x, \texttt{2020}), \relation{Contact}(\underline{y}, x).
\end{align*}
%
Finally, for the subtree $(\tau_C, \relation{Contact})$, the atom $\relation{Contact}(\underline{y}, x)$ is also unattacked in the corresponding subquery $\examplequery_{\tau_C}() \obtainedfrom \relation{Contact}(\underline{y}, x).
$
%
% \begin{align*}
% \end{align*}
%
Hence $(\tau, \relation{Employee})$ is a PPJT of $\examplequery$. \qed
\end{example}


\begin{figure}[t]
\begin{tikzpicture}[level distance=10em,
every node/.style = {line width=1pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right]
\tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=5mm, rectangle, rounded corners}};

\node (E) {$\textsf{Employee}(\underline{x}, y, z)$};
\node (M) [right of=E, node distance=3cm] {$\textsf{Manager}(\underline{y}, x, \texttt{2020})$};
\node (C) [right of=M, node distance=2.8cm] {$\textsf{Contact}(\underline{y}, x)$};

\path[->] (E) edge [line width=1pt] (M);
\path[->] (M) edge [line width=1pt] (C);

\node (box1) [draw=blue, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner xsep=3mm, inner ysep=4mm, rectangle, rounded corners,  fit = (E) (C)] {};
\node [above left = 0mm and -2mm of box1, draw=none,above] {{\color{blue} $\tau$}};                                
 \node (box2) [draw=red, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner xsep=2.2mm, inner ysep=2.6mm, rectangle, rounded corners,  fit = (M) (C)] {};    
\node [above left = 0.9mm and -2mm of box2, draw=none,above] {{\color{red} $\tau_M$}};                                   
\node (box3) [draw=brown, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner xsep=1.3mm, inner ysep=1.2mm, rectangle, rounded corners,  fit = (C) (C)] {};                                      
\node [above left = 2.2mm and -2mm of box3, draw=none,above] {{\color{brown} $\tau_C$}}; 

%%%%%%%%%%%%%% the query
%  \begin{scope}[xshift=3.5cm]
%         %E-diagram
% \node (E) {$\textsf{Employee}$};
% \node (M) [right of=E, node distance=2cm] {$\textsf{Manager}$};	
% \node (C) [above of=E, node distance=1cm]{$\textsf{Contact}$};	
% \path[->] (E) edge [line width=1pt] (M);
% \path[->] (E) edge [line width=1pt] (C);
% \node (box1) [draw=blue, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=2mm, rectangle, rounded corners,  fit = (E) (M) (C)] {};
% \node [above = 1mm of box1, draw=none]{\color{blue} attack graph of $\examplequery$};                                   
% \end{scope}

%  \begin{scope}[xshift=3.5cm, yshift=-2cm]
%         %E-diagram
% \node (M) {$\textsf{Manager}$};	
% \node (C) [right of=M, node distance=2cm]{$\textsf{Contact}$};	
% \node (box1) [draw=red, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=2mm, rectangle, rounded corners,  fit = (M) (C)] {};
%  \node [above = 1mm of box1, draw=none]{\color{red} attack graph of $\examplequery_{\tau_M}$};                                     
% \end{scope}

%  \begin{scope}[xshift=4.5cm, yshift=-4cm]
%         %E-diagram
% \node (C){$\textsf{Contact}$};	
% \node (box) [draw=brown, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=2mm, rectangle, rounded corners,  fit = (C)] {};   
%  \node [above = 1mm of box, draw=none]{\color{brown} attack graph of $\examplequery_{\tau_C}$};                                     
% \end{scope}
                                                        
%\node at (box1.north) [above, inner sep=3mm] {$\examplequery$};
\end{tikzpicture}
\caption{A pair-pruning join tree (PPJT) of the query $\examplequery$.
% \jef{I gues $w$ should read 2020.}
}
\label{fig:join-tree}
\end{figure}


\introparagraph{Which queries admit a PPJT?}
As we show next, having a PPJT is a sufficient condition for the existence of an \FO-rewriting. 

\begin{proposition}\label{prop:ppjt}
Let $q$ be an acyclic self-join-free BCQ. If $q$ has a PPJT, then $\cqa{q}$ admits an \FO-rewriting.
\end{proposition}

\reva{
Proposition~\ref{prop:ppjt} is proved in Appendix~\ref{sec:missing-proofs} of the extended version of this paper\zhiwei{TODO: we may need to add the link to the extended version}, in which we show that the if $q$ has a PPJT, then the attack graph of $q$ must be acyclic.}
We note that not all acyclic self-join-free BCQs with an acyclic attack graph have a PPJT, as demonstrated in the next example.

\begin{example}
\label{ex:noppjt}
Let $q() \obtainedfrom R(\underline{x, w}, y), S(\underline{y, w}, z), T(\underline{w}, z)$. The attack graph of $q$ is acyclic. The only join tree $\tau$ of $q$ is the path $R - S - T$. However, neither $(\tau, R)$ nor $(\tau, S)$ is a PPJT for $q$ since $R$ and $S$ are attacked in $q$; and $(\tau, T)$ is not a PPJT since in its subtree $(\tau', S)$, $S$ is attacked in the subquery that contains $R$ and $S$. \qed
\end{example}

\revb{Fuxman and Miller~\cite{FUXMAN2007610} identified a large class of queries called $\cforest$ that includes most queries with primary-key-foreign-key joins, path queries, and queries on a star schema, such as SSB and TPC-H \cite{DBLP:conf/tpctc/ONeilOCR09, poess2000new}.} This class covers most of the SPJ queries seen in practical settings. It can be shown that any acyclic join query in the class $\cforest$ has a PPJT. \revb{Therefore, most SPJ queries in practical settings that are already captured by $\cforest$ would have a PPJT.}

\begin{proposition}
\label{prop:cforest}
If an acyclic self-join-free BCQ $q$ is in $\cforest$, then $q$ has a pair-pruning join tree.
\end{proposition}

\revb{Moreover, for every SPJ query $q$ on two tables, if $\cqa{q}$ is in \FO, then $q$ must have a PPJT, but is not necessarily in $\cforest$. Indeed, every CQ $q$ on two atoms is acyclic and has a join tree $\tau$, and since $\cqa{q}$ is in \FO, there is a reifiable atom $R$ in $q$ \zhiwei{We no longer define the term reifiable - need to rephrase here}, and thus $(\tau, R)$ is a PPJT of $q$. The query $q_5$ in Section~\ref{sec:synthetic} has two atoms but is not in $\cforest$. This \jef{What is ``This'' referring to? Do you mean something like: It turns out that most SPJ queries on two tables in realistic workloads have a PPJT.} captures most SPJ queries on two tables in realistic workloads.}


\jef{Consider the following.}
\jef{
The inverse of Propostion~\ref{prop:cforest} is not true, and already fails for queries on two tables, which are acyclic by definition. For example, the query $q_5$ in Section~\ref{sec:synthetic} has a PPJT but is not in $\cforest$. It turns out that most SPJ queries on two tables in realistic workloads have a PPJT. 
}
\xiating{My intention here is to emphasize that PPJT captures a very specific class of CQs: SPJ queries on two tables that are in \FO. In this case $\cqa{q}$ is in \FO~iff $q$ has a PPJT. This also happens to show that the inverse of Proposition~\ref{prop:cforest} fails.}
%\xiating{
%Perhaps we should enumerate all CQs on some fixed schema via the Bell number approach and show some statistics? Or we can argue that the following conjecture also captures a ``large'' class of CQs.
%\begin{conjecture}
%Let $q$ be an acyclic self-join-free BCQ whose attack graph is acyclic. If all attacks in $q$ are weak, then $q$ has a pair-pruning join tree.
%\end{conjecture}
%Note that this would be a stronger statement than Proposition~\ref{prop:cforest}, since if $q$ is in $\cforest$, then all attacks in $q$ must be weak.
%}


\introparagraph{How to find a PPJT.}
For any acyclic self-join-free BCQ $q$, we can check whether $q$ admits a PPJT via a brute-force search over all possible join trees and roots. If $q$ involves $n$ relations, then there are at most $n^{n-1}$ candidate rooted join trees for PPJT ($n^{n-2}$ join trees and for each join tree, $n$ choices for the root). \revb{For the data complexity of $\cqa{q}$, this exhaustive search runs in constant time since we assume $n$ is a constant. In practice, the search cost is acceptable for most join queries that do not involve too many tables.}

% For acyclic queries not involving joins between primary keys, a PPJT can be constructed efficiently without the need of an exhaustive search, shown in Appendix~\ref{sec:no-key-containment}. \xiating{Removed the proposition for no key containment.}
% \jef{The foregoing statement is unclear. Here is a suggestion.}
% \jef{
%  
Appendix~\ref{sec:no-key-containment} of the extended version of this paper\zhiwei{TODO: add reference} shows that the foregoing brute-force search for $q$ can be optimized to run in polynomial time when~$q$ has an acyclic attack graph and, \revb{when expressed as a rule}, does not contain two distinct body atoms $R(\underline{\vec{x}},\vec{y})$ and $S(\underline{\vec{u}},\vec{w})$ such that every variable occurring in $\vec{x}$ also occurs in~$\vec{u}$. Most queries we observe and used in our experiments fall under this category.
% }
% \jef{Note that the foregoing statement looks asymmetric in $\vec{x}$ and $\vec{u}$, but that is fine since the roles of $R$ and $S$ can be switched.}


\introparagraph{Main Result.} 
We previously showed that the existence of a PPJT implies an \FO-rewriting that computes the consistent answers. Our main result shows that it also leads to an efficient algorithm that runs in linear time.

\begin{theorem}
\label{thm:main:boolean}
Let $q$ be an acyclic self-join-free Boolean CQ that admits a PPJT, and $\db$ be a database instance of size $N$. Then, there exists an algorithm for $\cqa{q}$ that runs in time $O(N)$.
\end{theorem}

It is worth contrasting our result with Yannakakis' algorithm, which computes the result of any acyclic Boolean CQ also in linear time $O(N)$~\cite{DBLP:conf/vldb/Yannakakis81}. Hence, the existence of a PPJT implies that computing $\cqa{q}$ will have the same asymptotic complexity. 
\reva{Theorem~\ref{thm:main:boolean} will be proved in Section~\ref{sec:datalog} and~\ref{sec:correctness-boolean}, where we present the \FO-rewriting rules and show they run in linear time, and prove their correctness respectively.}

\introparagraph{Disconnected CQs.}
Every disconnected BCQ $q$ can be written as $q = q_1, q_2, \dots, q_n$ where $\var{q_i} \cap \var{q_j} = \emptyset$ for $1 \leq i < j \leq n$ and each $q_i$ is connected. If each $q_i$ has a PPJT, then $\cqa{q}$ can be solved by checking whether the input database is a ``yes''-instance for each $\cqa{q_i}$, by Lemma~B.1 of \cite{DBLP:conf/pods/KoutrisOW21}.



\subsection{The Rewriting Rules}
\label{sec:datalog}

We now show how to produce an efficient rewriting. We will use Datalog syntax to describe the rewriting, since it will simplify the exposition. In Section~\ref{sec:implementation}, we will discuss how to translate the Datalog program to SQL.

%\begin{figure}[h!]
%    \centering
%    \tikz\path (0,0) node[draw, text width=.4\textwidth, rectangle, inner xsep=20pt, inner ysep=10pt]{
%        \begin{minipage}[t!]{\textwidth}
%            {\sc Procedure}: $\textsc{PPJT-Rewriting}(\tau, R)$
%            \\
%            {\sc Input}: the PPJT $(\tau, R)$ of $q$
%            \\
%            {\sc Output}: a Datalog program computing $\goodkey{R}{q}{\db}$
%            \begin{tabbing}
%                Aaa\=aaA\=Aaa\=Aaa\=Aaa\=AAAAAAAAAAAAAAAAAAAAAAAAA\=A \kill
%               1. \> $\textsc{Self-Pruning}(R)$
%               \\
%               2. \> {\bf for each } child node $S$ of $R$ in $\tau$ {\bf do } 
%               \\
%               3. \>\> $\textsc{PPJT-Rewriting}(\tau, S)$
%               \\
%               4. \>\>  $\textsc{Pair-Pruning}(R, S)$
%               \\
%               5. \> $\textsc{Exit-Rule}(R)$
%            \end{tabbing}  
%        \end{minipage}
%    };
%    \caption{}
%\end{figure}

%%%%%%%%%%%%%%%%%% embedding %%%%%%%%%%%%%%%%%%5
\begin{figure*}[t]
\small
\subfloat[Yannakakis' algorithm]{
     \begin{tikzpicture}[level distance=10em,
every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
\tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=5mm, rectangle, rounded corners}};

\node (E-exit) [draw=none] {
     $\relation{Employee}_{\mathsf{join}}() \obtainedfrom \relation{Employee}(x, y, z), \relation{Manager}_{\mathsf{join}}(y, x).$};

\node (E-data) [below right= 1 cm and 1.4cm of E-exit.west, anchor=west, draw=none] {
$\textsf{Employee}_{\mathsf{join}}$ is nonempty.
};



\node (M-exit) [below = 2 cm of E-exit.west, anchor=west, draw=none]{     
      $\relation{Manager}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \relation{Contact}_{\mathsf{join}}(y, x).$}; 

\node (M-data) [below right= 1.65cm and 1.4cm of M-exit.west, anchor=west, draw=none]{     
\begin{tabular}{|c c}
 $\textsf{Manager}_{\mathsf{join}}$ & \\
 \hline
{Boston} & {0011}  \\
Chicago & 0022 \\
{LA} & {0034}  \\
{LA} & {0037}  \\
New York & 0022
\end{tabular}
}; 


\node (C-exit) [below =3.4 cm of M-exit.west, anchor=west, draw=none] {
     $\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x).$};

\node (C-data) [below right=1.8 cm and 1.4cm of C-exit.west, anchor=west, draw=none] {
\begin{tabular}{|c c}
$\textsf{Contact}_{\mathsf{join}}$ & \\
\hline
{Boston} & {0011}\\
{Boston} & {0022} \\
Chicago &  0022 \\
{LA} & {0034}  \\
{LA} & {0037} \\
New York & 0022 
\end{tabular}
};




\path[->] (E-exit.south west)+(1,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
{} ($(1,0.2)+(M-exit.north west)$) ;


\path[->] (M-exit.south west)+(1,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
{} ($(C-exit.north west)+(1,0.2)$) ;

\node (box1) [draw=blue, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (E-exit)] {};
 
\node (box2) [draw=red, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (M-exit)] {};    

\node (box3) [draw=brown, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (C-exit)] {};                                      
% \node [below=0.4cm of box3, white] {};
% \node [right = 13mm of box1, above = 1mm of box1, draw=none] {{\color{blue} $\relation{Employee}(\underline{x},y,z)$}};
% \node [right = 15mm of box2, above = 1mm of box2, draw=none] {{\color{red} $\relation{Manager}(\underline{y},x,w)$}}; 
% \node [right = 20mm of box3, above = 1mm of box3, draw=none] {{\color{brown} $\relation{Contact}(\underline{y},x)$}}; 
                                                        
\end{tikzpicture}

}
\quad
\subfloat[PPJT]{
     \begin{tikzpicture}[level distance=10em,
every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
\tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=5mm, rectangle, rounded corners}};

\node (E-exit) [draw=none] {
     \textbf{R4: }$\relation{Employee}_{\mathsf{join}}() \obtainedfrom \relation{Employee}(x, y, z), \lnot \fk{\relation{Employee}}(x).$};
\node (E-self) [below = 0.6cm of E-exit.west, anchor=west, draw=none] {    
     \textbf{R3: }$\fk{\relation{Employee}}(x)  \obtainedfrom \relation{Employee}(x, y, z), \lnot \relation{Manager}_{\mathsf{join}}(y, x).$};

\node (E-data) [below right =1.1 cm and 1.2cm of E-self.west, anchor=west, draw=none] {
\begin{tabular}{c c}
\begin{tabular}{|c c}
$\fk{\textsf{Employee}}$ & \\
\cline{1-1}
0011 & \multirow{2}{0.1cm}{\textbf{R3}}\\
0034 &  \\
\end{tabular}
&
\begin{tabular}{c}
$\textsf{Employee}_{\mathsf{join}}$ is nonempty.
\end{tabular}
\end{tabular}
};

\node (M-exit) [below = 2.1 cm of E-self.west, anchor=west, draw=none]{     
      \textbf{R4: }$\relation{Manager}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \lnot \fk{\relation{Manager}}(y).$}; 
     
\node (M-self) [below =0.9cm of M-exit.west, anchor=west, draw=none]{ 
     % \node (M-self) [below =1cm of M-exit.west, anchor=west, draw=none]{ 
%       $\begin{aligned}
%       &\fk{\relation{Manager}}(z_1)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq 2020.  \\
%       & \fk{\relation{Manager}}(z)   \obtainedfrom \relation{Manager}(z, x, 2020), \relation{Manager}(z, z_1, z_2), z_1 \neq x.
%       \end{aligned}$};
     $\begin{aligned}
     \textbf{R3: }& \fk{\relation{Manager}}(y)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \lnot \relation{Contact}_{\mathsf{join}}(y, x). \\
     \textbf{R2: }&\fk{\relation{Manager}}(y)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \relation{Manager}(y, z_1, \texttt{2020}), z_1 \neq x. \\
     \textbf{R1: }&\fk{\relation{Manager}}(z_1)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq 2020.
     \end{aligned}$
     };


\node (M-data) [below right=1.55 cm and 1.15cm of M-self.west, anchor=west, draw=none] {
\begin{tabular}{c c}
\begin{tabular}{|c c}
$\fk{\textsf{Manager}}$ & \\
\cline{1-1}
{Boston} & \textbf{R1, R3}\\
{LA} &  \textbf{R2, R3}\\
\end{tabular}
&
\begin{tabular}{|c c}
$\textsf{Manager}_{\mathsf{join}}$ & \\
\hline
Chicago &  0022 \\
New York & 0022 
\end{tabular}
\end{tabular}
};


\node (C-exit) [below =3.6 cm of M-exit.west, anchor=west, draw=none] {
     \textbf{R4: }$\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x), \lnot \fk{\relation{Contact}}(y).$};

\node (C-self) [below = 0.6cm of C-exit.west, anchor = west, draw=none] {
     \textbf{R2: }$\fk{\relation{Contact}}(y)  \obtainedfrom \relation{Contact}(y, x), \relation{Contact}(y, z_1), z_1 \neq x.$};


\node (C-data) [below right=1cm and 1.1cm of C-self.west, anchor=west, draw=none] {
\begin{tabular}{c c}
\begin{tabular}{|c c}
$\fk{\relation{Contact}}$ \\
\cline{1-1}
{Boston}& \multirow{2}{0.1cm}{\textbf{R2}} \\
{LA}
\end{tabular}
&
\begin{tabular}{|c c}
$\textsf{Contact}_{\mathsf{join}}$ & \\
\hline
Chicago &  0022 \\
New York & 0022 
\end{tabular}
\end{tabular}
};


\path[->] (E-self.south west)+(1,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
{} ($(1,0.2)+(M-exit.north west)$) ;

\path[->] (M-self.south west)+(1,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
{} ($(C-exit.north west)+(1,0.2)$) ;

\node (box1) [draw=blue, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (E-exit) (E-self)] {};

 \node (box2) [draw=red, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (M-exit) (M-self)] {};    

\node (box3) [draw=brown, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (C-exit) (C-self)] {};                                      
% \node [right = 13mm of box1, draw=none, above] {{\color{blue} $\relation{Employee}(\underline{x},y,z)$}}; 
% \node [right = 15mm of box2, draw=none, above] {{\color{red} $\relation{Manager}(\underline{y},x,w)$}}; 
% \node [right = 10mm of box3, draw=none, above] {{\color{brown} $\relation{Contact}(\underline{y},x)$}}; 
                                                        
\end{tikzpicture}
\label{fig:example-rewriting}
}
\caption{The non-recursive Datalog program for evaluating $\examplequery$ (a) and $\cqa{\examplequery}$ (b), together with an example execution on the \textbf{Company} database in Figure~\ref{fig:incon_db_example}.}

\end{figure*}


\begin{figure*}[t]
\small
\subfloat[Yannakakis' algorithm]{
     \begin{tikzpicture}[level distance=10em,
every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
\tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=5mm, rectangle, rounded corners}};

\node (E-exit) [draw=none] {
     $\relation{Employee}_{\mathsf{join}}() \obtainedfrom \relation{Employee}(x, y, z), \relation{Manager}_{\mathsf{join}}(y, x).$};

\node (M-exit) [below = 2.25 cm of E-exit.west, anchor=west, draw=none]{     
      $\relation{Manager}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \relation{Contact}_{\mathsf{join}}(y, x).$}; 

\node (C-exit) [below =2.3 cm of M-exit.west, anchor=west, draw=none] {
     $\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x).$};


\path[->] (E-exit.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
{} ($(3,0.2)+(M-exit.north west)$) ;


\path[->] (M-exit.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
{} ($(C-exit.north west)+(3,0.2)$) ;

\node (box1) [draw=blue, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (E-exit)] {};
 
\node (box2) [draw=red, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (M-exit)] {};    

\node (box3) [draw=brown, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (C-exit)] {};                                      
\node [below=0.4cm of box3, white] {};
% \node [right = 13mm of box1, above = 1mm of box1, draw=none] {{\color{blue} $\relation{Employee}(\underline{x},y,z)$}};
% \node [right = 15mm of box2, above = 1mm of box2, draw=none] {{\color{red} $\relation{Manager}(\underline{y},x,w)$}}; 
% \node [right = 20mm of box3, above = 1mm of box3, draw=none] {{\color{brown} $\relation{Contact}(\underline{y},x)$}}; 
                                                        
\end{tikzpicture}

}
\quad
\subfloat[PPJT]{
     \begin{tikzpicture}[level distance=10em,
every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
\tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=5mm, rectangle, rounded corners}};

\node (E-exit) [draw=none] {
     \textbf{R4: }$\relation{Employee}_{\mathsf{join}}() \obtainedfrom \relation{Employee}(x, y, z), \lnot \fk{\relation{Employee}}(x).$};
\node (E-self) [below = 0.6cm of E-exit.west, anchor=west, draw=none] {    
     \textbf{R3: }$\fk{\relation{Employee}}(x)  \obtainedfrom \relation{Employee}(x, y, z), \lnot \relation{Manager}_{\mathsf{join}}(y, x).$};

\node (M-exit) [below = 1.6 cm of E-self.west, anchor=west, draw=none]{     
      \textbf{R4: }$\relation{Manager}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \lnot \fk{\relation{Manager}}(y).$}; 
     
\node (M-self) [below =0.9cm of M-exit.west, anchor=west, draw=none]{ 
     % \node (M-self) [below =1cm of M-exit.west, anchor=west, draw=none]{ 
%       $\begin{aligned}
%       &\fk{\relation{Manager}}(z_1)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq 2020.  \\
%       & \fk{\relation{Manager}}(z)   \obtainedfrom \relation{Manager}(z, x, 2020), \relation{Manager}(z, z_1, z_2), z_1 \neq x.
%       \end{aligned}$};
     $\begin{aligned}
     \textbf{R3: }& \fk{\relation{Manager}}(y)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \lnot \relation{Contact}_{\mathsf{join}}(y, x). \\
     \textbf{R2: }&\fk{\relation{Manager}}(y)  \obtainedfrom \relation{Manager}(y, x, \texttt{2020}), \relation{Manager}(y, z_1, \texttt{2020}), z_1 \neq x. \\
     \textbf{R1: }&\fk{\relation{Manager}}(z_1)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq 2020. 
     \end{aligned}$
     };

\node (C-exit) [below =2 cm of M-self.west, anchor=west, draw=none] {
     \textbf{R4: }$\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x), \lnot \fk{\relation{Contact}}(y).$};

\node (C-self) [below = 0.6cm of C-exit.west, anchor = west, draw=none] {
     \textbf{R2: }$\fk{\relation{Contact}}(y)  \obtainedfrom \relation{Contact}(y, x), \relation{Contact}(y, z_1), z_1 \neq x.$};

\path[->] (E-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
{} ($(3,0.2)+(M-exit.north west)$) ;

\path[->] (M-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
{} ($(C-exit.north west)+(3,0.2)$) ;

\node (box1) [draw=blue, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (E-exit) (E-self)] {};

 \node (box2) [draw=red, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (M-exit) (M-self)] {};    

\node (box3) [draw=brown, line width=1pt,
                               dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                inner sep=1mm, rectangle, rounded corners,  fit = (C-exit) (C-self)] {};                                      
% \node [right = 13mm of box1, draw=none, above] {{\color{blue} $\relation{Employee}(\underline{x},y,z)$}}; 
% \node [right = 15mm of box2, draw=none, above] {{\color{red} $\relation{Manager}(\underline{y},x,w)$}}; 
% \node [right = 10mm of box3, draw=none, above] {{\color{brown} $\relation{Contact}(\underline{y},x)$}}; 
                                                        
\end{tikzpicture}
\label{fig:example-rewriting}
}
\caption{The non-recursive Datalog program for evaluating $\examplequery$ and $\cqa{\examplequery}$.}

\end{figure*}

\begin{figure*}
\small
\begin{tabular}{c c c}
\begin{tabular}{|c c c c}
\multicolumn{4}{c}{\textsf{Employee}} \\
\primarykey{\textsf{employee\_id}} & \textsf{office\_city} & \textsf{wfh\_city} & \\
\cdashline{1-3}
{\color{red} 0011} & Boston &Boston & \multirow{3}{0.05cm}{\textbf{R3}} \\
{\color{red} 0011} & Chicago & New York & \\
{\color{red} 0011} & Chicago & Chicago & \\
\cdashline{1-3}
0022 & New York & New York & \multirow{2}{0.05cm}{\textbf{R4}} \\
0022 & Chicago & Chicago & \\
\cdashline{1-3}
{\color{red} 0034} & Boston & New York & \multirow{1}{0.05cm}{\textbf{R3}}
\end{tabular}
&
\begin{tabular}{|c c c c}
\multicolumn{4}{c}{\textsf{Manager}} \\
\primarykey{\textsf{office\_city}} & \textsf{manager\_id} & \textsf{start\_year} & \\
\cdashline{1-3}
{\color{red} Boston} & {0011} & {2020} & \multirow{2}{0.85cm}{\textbf{R1, R3}}\\
{\color{red} Boston} & {0011} & {2021} & \\
\cdashline{1-3}
{\color{blue} Chicago} & {\color{blue} 0022} & 2020 & \multirow{1}{0.85cm}{\textbf{R4}} \\
\cdashline{1-3}
{\color{red} LA} & {0034} & {2020} & \multirow{2}{0.85cm}{\textbf{R2, R3}}\\
{\color{red} LA} & {0037} & {2020} & \\
\cdashline{1-3}
{\color{blue} New York} & {\color{blue} 0022} & 2020 & \multirow{1}{0.85cm}{\textbf{R4}}
\end{tabular}
&
\begin{tabular}{|c c c}
\multicolumn{3}{c}{\textsf{Contact}} \\
\primarykey{\textsf{office\_city}} & \textsf{contact\_id} & \\
\cline{1-2}
{\color{red} Boston} & {0011} & \multirow{2}{0.05cm}{\textbf{R2}} \\
{\color{red} Boston} & {0022} & \\
\cdashline{1-2}
{\color{blue} Chicago} &  {\color{blue} 0022} & \multirow{1}{0.05cm}{\textbf{R4}} \\
\cdashline{1-2}
{\color{red} LA} & {0034} & \multirow{2}{0.05cm}{\textbf{R2}} \\
{\color{red} LA} & {0037} & \\
\cdashline{1-2}    
{\color{blue} New York} & {\color{blue} 0022} & \multirow{1}{0.05cm}{\textbf{R4}}
\end{tabular}
\end{tabular}
\caption{Presentation of the execution of the rewriting rules of Figure~\ref{fig:example-rewriting} on the \textbf{Company} database in Figure~\ref{fig:incon_db_example}. Each block of a table named~$\relation{R}$ is annotated with all the rules fired on it.  Red-colored primary-key values indicate blocks added to $\fk{\relation{R}}$, which are thus pruned away.  
Blue-colored  attribute values will occur in $\relation{R}_{\mathsf{join}}$.
%%%
Recall that the original query is $\examplequery() \obtainedfrom \relation{Employee}(\underline{x}, y, z), \relation{Manager}(\underline{y}, x, \texttt{2020}), \relation{Contact}(\underline{y}, x)$.}
\label{fig:example-run}
\end{figure*}


% ***************************** OLD PPJT REWRITING BELOW
% \begin{figure*}[t]

% \begin{tikzpicture}[level distance=10em,
% every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
% brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
% \tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=5mm, rectangle, rounded corners}};

% \node (E-exit) [draw=none] {
%      $\relation{Employee}_{\mathsf{join}}() \obtainedfrom \relation{Employee}(x, y, y), \lnot \fk{\relation{Employee}}(x).$};
% \draw [brace]  (E-exit.south west) -- (E-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};  

% \node (E-self) [below = 0.75cm of E-exit.west, anchor=west, draw=none] {   
%      $\fk{\relation{Employee}}(z_1)  \obtainedfrom \relation{Employee}(z_1, z_2, z_3), z_3 \neq z_2. $};
% \draw [brace]  (E-self.south west) -- (E-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

% \node (M-exit) [below = 2 cm of E-self.west, anchor=west, draw=none]{       
%       $\relation{Manager}_{\mathsf{join}}(z, x)  \obtainedfrom \relation{Manager}(z, x, 2020), \lnot \fk{\relation{Manager}}(z).$}; 
% \draw [brace]  (M-exit.south west) -- (M-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};  
      
% \node (M-self) [below =1cm of M-exit.west, anchor=west, draw=none]{ 
%       $\begin{aligned}
%       &\fk{\relation{Manager}}(z_1)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq 2020.  \\
%       & \fk{\relation{Manager}}(z)   \obtainedfrom \relation{Manager}(z, x, 2020), \relation{Manager}(z, z_1, z_2), z_1 \neq x.
%       \end{aligned}$};
% \draw [brace]  (M-self.south west) -- (M-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

% \node (C-exit) [below =2 cm of M-self.west, anchor=west, draw=none] {
%      $\relation{Contact}_{\mathsf{join}}(z, x)  \obtainedfrom \relation{Contact}(z, x), \lnot \fk{\relation{Contact}}(z).$};
% \draw [brace]  (C-exit.south west) -- (C-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};

% \node (C-self) [below = 0.75cm of C-exit.west, anchor = west, draw=none] {
%      $\fk{\relation{Contact}}(z)  \obtainedfrom \relation{Contact}(z, x), \relation{Contact}(z, z_1), z_1 \neq x.$};
% \draw [brace]  (C-self.south west) -- (C-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};


% \path[->] (E-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
% {$\fk{\relation{Employee}}(x)  \obtainedfrom \relation{Employee}(x, z, z), \lnot \relation{Manager}_{\mathsf{join}}(z, x).$} ($(3,0.2)+(M-exit.north west)$) ;

% \draw [brace]   (PP.north east) -- (PP.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

% \path[->] (M-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
% {$ \fk{\relation{Manager}}(z)  \obtainedfrom \relation{Manager}(z, x, 2020), \lnot \relation{Contact}_{\mathsf{join}}(z, x). $} ($(C-exit.north west)+(3,0.2)$) ;

% \draw [brace]   (PP2.north east) -- (PP2.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

% \node (box1) [draw=blue, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (E-exit) (E-self)] {};
% \node [right = 13mm of box1, draw=none, above] {{\color{blue} $\relation{Employee}(\underline{x},z,z)$}}; 

%  \node (box2) [draw=red, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (M-exit) (M-self)] {};    
% \node [right = 15mm of box2, draw=none, above] {{\color{red} $\relation{Manager}(\underline{z},x,2020)$}}; 

% \node (box3) [draw=brown, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (C-exit) (C-self)] {};                                      
% \node [right = 10mm of box3, draw=none, above] {{\color{brown} $\relation{Contact}(\underline{z},x)$}}; 
                                                        
% \end{tikzpicture}
% \caption{The non-recursive Datalog program produced for $\cqa{\examplequery}$.}
% \label{fig:example-rewriting}
% \end{figure*}

\revb{%For a BCQ $q$ with a PPJT $(\tau, R)$,
%
%$$\badkey{R}{q}{\db} := R_{\mathsf{key}}(q,\db) \setminus \goodkey{R}{q}{\db}.$$ 
%We will use $\gk{R}$ and $\bk{R}$ to denote the sets $\goodkey{R}{q}{\db}$ and $\badkey{R}{q}{\db}$ respectively. 
To describe the rewriting of a BCQ $q$ with a PPJT $(\tau, R)$, we will need two predicates for every atom $S$ in the tree (let $T$ be the unique parent of $S$ in $\tau$):}
%
\begin{itemize}
\item the predicate $\fk{S}$ has arity equal to $|\key{S}|$ and collects the primary-key values of the $S$-table that cannot contribute to a consistent answer for $q$~\footnote{The \textsf{f} in $\textsf{fkey}$ is for ``\underline{f}alse key''. 
% We want to distinguish it from ``bad key'' because the latter is natural to be interpreted as ``not good key'', but in fact the set $\fk{S}$ computed by the rules (sometimes strictly) contains the ``not good keys''.
}; and
%Rule~\ref{rule:self-pruning} and Rule~\ref{rule:bad-key-simplified} computes ``not good keys'' for $\cqa{q_{\tau_S}}$, and Rule~\ref{rule:good-join} computes the additional keys, possibly in $\gk{S}$ of $\cqa{q_{\tau_S}}$, that should be excluded. 
\item the predicate $\jk{S}$ has arity equal to $|\var{S} \cap \var{T}|$ and collects the values for these variables in the $S$-table that may contribute to a consistent answer.
\end{itemize}

The rewriting algorithm traverses the PPJT recursively starting from the root of the tree.
% \jef{I changed the code. Please check.}
%
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\begin{algorithm}[!ht]
\DontPrintSemicolon
  
  \KwInput{PPJT $(\tau, R)$ of $q$}
  \KwOutput{a Datalog program $P$ deciding $\cqa{q}$}

  $P:=\emptyset$ \; 
  $P:=P\cup\textsc{Self-Pruning}(R)$ \;
  \ForEach{child node $S$ of $R$ in $\tau$}{
  $P:=P\cup\textsc{PPJT-Rewriting}(\tau, S)$ \;
  $P:=P\cup\textsc{Pair-Pruning}(R, S)$ \;
  }
  $P:=P\cup\textsc{Exit-Rule}(R)$ \;
  \Return $P$ \;
\caption{$\textsc{PPJT-Rewriting}(\tau, R)$}
    \label{fig:ppjt}
\end{algorithm}

\revb{At a high level, the procedure \textsc{Self-Pruning}($R$) finds the keys of $R$ whose blocks contain some fact that violates the local selection condition, yielding $\fk{R}$; and procedure \textsc{Pair-Pruning}($R, S$) computes the keys of $R$ whose blocks contain some fact that does not satisfy the joining (J) condition with its child $S$ in $(\tau, R)$.} 
Figure~\ref{fig:example-rewriting} depicts how each step generates the rewriting rules for  $\examplequery$.

We now describe how each step is implemented in detail. 

\smallskip
\noindent \underline{\textsc{Self-Pruning}($R$)}: Let $R(\underline{x_1, \dots x_k}, x_{k+1}, \dots, x_n)$, where $x_i$ can be a variable or a constant. The first rule finds the primary-key values of the $R$-table that can be pruned because of the local selection conditions imposed on $R$. \revb{Intuitively, if a block contains some fact that violates the local selection condition, then the repair containing that fact will not satisfy the query condition, and thus that block can be safely removed.}

%$$\gvec{y}[i] = \begin{cases}
%\vec{y}[i] & \text{ if $\vec{y}[i] \in \var{\vec{y}} \setminus \var{\vec{x}}$ and} \\
%& \hspace{1cm} \text{there is no $j < i$ with $\vec{y}[j] = \vec{y}[i]$} \\
%z_i & \text{ otherwise, where $z_i$ is a fresh variable.}
%\end{cases}
%$$

\begin{rules}
\label{rule:self-pruning}
If $x_i = c$ for some constant $c$, we add the rule 
\begin{align*}
\fk{R}(z_1, \dots, z_k) \obtainedfrom R(z_1, \dots, z_n), z_i \neq c.
\end{align*}
If for some variable $x_i$ there exists $j<i$ with $x_i = x_j$, we add the rule
\begin{align*}
\fk{R}(z_1, \dots, z_k) \obtainedfrom R(z_1, \dots, z_n), z_i \neq z_j.
\end{align*}
Here, $z_1, \dots, z_n$ are fresh distinct variables.
\end{rules}

The second rule finds the primary-key values of the $R$-table that can be pruned because $R$ joins with its parent $T$ in the tree. The underlying intuition is that if some $R$-block of the input database contains two tuples that disagree on a non-key position that is used in an equality-join with~$T$, then for every given $T$-tuple~$t$, we can pick an $R$-tuple in that block that does not join with $t$. \revb{Informally, if all facts in an inconsistent block in $R$ can contribute to a consistent answer, then all these facts must agree on the joining attributes with~$T$, the parent of $R$ in the PPJT, because $R$ does not attack $T$ in~$q_{\tau_T}$.}

%Our first step is to keep only those $S$-blocks of the input such that for every $i\in\{1,\dots,\card{\vec{v}}\}$, if a variable of $\var{\vec{w}}$ occurs at position~$i$ in $\vec{v}$, then all facts in the block agree on position~$\card{\vec{u}}+i$.


\begin{rules}
\label{rule:good-join}
 For each variable $x_i$ with $i>k$ (so in a non-key position) such that $x_i \in \var{T}$, we produce a rule
\begin{align*}
     \fk{R}(x_1, \dots, x_k)  \obtainedfrom & R(x_1, \dots, x_k, x_{k+1}, \dots, x_n), \\
     & R(x_1, \dots, x_k, z_{k+1}, \dots,  z_k), z_i \neq x_i.
\end{align*}
where $z_{k+1}, \dots, z_n$ are fresh variables.
%Next, produce a rule
%\begin{align}
%     S_{\mathsf{gkey-join}}(\vec{u}) & \obtainedfrom \gk{S}(\vec{u}), \lnot S_{\mathsf{disagree-join}}(\vec{u}). 
%\end{align}
\end{rules}

\begin{example}
% The self-pruning step at the PPJT $(\tau, \relation{Employee})$ produces one rule (from Rule~\ref{rule:self-pruning}) since the atom 
% $\relation{Employee}(\underline{x},z,z)$ has one variable that occurs twice.  
% %\begin{align*}
% %     \fk{\relation{Employee}}(x) \obtainedfrom \relation{Employee}(\underline{x}, y, z_2), z_2 \neq y.
% %\end{align*}
% When executed on the \database{Company} database, keys $0011$ and $0034$ would be added to $\fk{\relation{Employee}}$.
The self-pruning phase on$(\tau_M, \relation{Manager})$ produces one rule using Rule~\ref{rule:self-pruning}. When executed on the \database{Company} database, the key Boston is added to $\fk{\relation{Manager}}$.

Finally, the self-pruning phase on the PPJT $(\tau_C, \relation{Contact})$ produces one rule using Rule~\ref{rule:good-join} (here $x$ is the non-key join variable). Hence, the keys Boston and LA will be added to $\fk{\relation{Contact}}$. \qed
\end{example}


\smallskip
\noindent \underline{\textsc{Pair-Pruning}($R,S$)}: Suppose that $q$ contains the atoms $R(\underline{\vec{x}}, \vec{y})$ and $S(\underline{\vec{u}}, \vec{v})$, where the $S$-atom is a child of the $R$-atom in the PPJT. Let $\vec{w}$ be a sequence of distinct variables containing all (and only) variables in $\var{R} \cap \var{S}$.
%be an arbitrary sequence of all distinct joining variables between $R(\underline{\vec{x}}, \vec{y})$ and $S(\underline{\vec{u}}, \vec{v})$. 
%Let $\tau$ be the subtree rooted at $S$. 


The pair-pruning step introduces one rule, which uses the fact that a key $\vec{c}\in R_{\mathsf{key}}(q,\db)$ can be pruned if there is a fact $R(\underline{\vec{c}}, \vec{d})$ that does not join with any fact in $S_{\mathsf{join}}(\vec{w})$. The intuition is that the fact $R(\underline{\vec{c}}, \vec{d})$ will not contribute to any consistent answer of $q$ in any repair containing it. 
% This idea is formalized in Lemma~\ref{lemma:pair-pruning}.

% The pair-pruning step introduces one rule, which uses the fact that, by item~\ref{it:pair-pruning}, a key $\vec{c}\in R_{\mathsf{key}}(q,\db)$ can be pruned if there is a fact $R(\underline{\vec{c}}, \vec{d})$ such that for every "good" key $\vec{s}$ from the $S$-table,  $R(\underline{\vec{c}}, \vec{d})$ does not join with any fact in $S(\underline{\vec{s}},*)$.

%Next, note that for all blocks that have passed the filtering condition of the pair-pruning step, all facts in the $S$-block $S(\underline{\vec{s}}, *)$ agree on each position at which a variable of $\vec{w}$ occurs in $S(\underline{\vec{u}},\vec{v})$. 
%Hence by item~\ref{it:pair-pruning}, a key $\vec{c}\in R_{\mathsf{key}}(q,\db)$ is a bad key if there is a fact $R(\underline{\vec{c}}, \vec{d})$ such that for every $\vec{s} \in S_{\mathsf{goodkey-join}}$,  $R(\underline{\vec{c}}, \vec{d})$ does not join with any fact in $S(\underline{\vec{s}},*)$. By construction, if $R(\underline{\vec{c}}, \vec{d})$ joins with some fact in $S(\underline{\vec{s}},*)$, then it joins with every fact in $S(\underline{\vec{s}},*)$.

\begin{rules}
\label{rule:bad-key-simplified}
Add the rule
\begin{align*}
     \fk{R}(\vec{x}) & \obtainedfrom R(\vec{x}, \vec{y}), \lnot S_{\mathsf{join}}(\vec{w}),
\end{align*}
where the rules for $S_{\mathsf{join}}$ will be defined in Rule~\ref{rule:return-simplified}.
\end{rules}
The rule is safe because every variable in $\vec{w}$ occurs in $R(\vec{x}, \vec{y})$.


%In implementation, we find all blocks $\vec{s} \in \goodkey{S}{q_\tau}{\db}$ such that there exist two facts $S(\vec{s}, \vec{t_1})$ and $S(\vec{s}, \vec{t_2})$ that disagree on $\var{\vec{w}}$. 
%For the atom $S(\underline{\vec{u}}, \vec{v})$, we introduce the vector $\jvec{v}$ as follows, {for $1\leq i\leq\card{\vec{v}}$}:
%$$\jvec{v}[i] = \begin{cases}
%z_i & \text{ if $\vec{v}[i] \in \var{\vec{w}} \setminus \var{\vec{u}}$.} \\
%\vec{v}[i] & \text{ otherwise,}
%\end{cases}
%$$
%{where $z_{1},\dots,z_{\card{\vec{v}}}$ are fresh variables.}
%\jef{
%I understand that $\jvec{v}$ is obtained from $\vec{v}$ be putting a fresh variable at every position at which a variable of $\var{\vec{w}} \setminus \var{\vec{u}}$ occurs.
%}


\begin{example}
Figure~\ref{fig:example-rewriting} shows the two pair-pruning rules generated (in general, there will be one pair-pruning rule for each edge in the PPJT). In both cases, the join variables are $\{y,x\}$. \qed
\end{example}


\smallskip
\noindent \underline{\textsc{Exit-Rule}($R$)}: Suppose that $q$ contains $R(\underline{\vec{x}}, \vec{y})$. Let $\vec{w}$ be a sequence of distinct variables containing all (and only) variables in $R$ and its parent node in $\tau$ (so the join variables). If $R$ is the root node, then $\vec{w}$ is the empty vector.
\revb{The exit rule removes the pruned blocks of $R$ and performs a projection on the join attributes $\vec{w}$ with its parent, which will be used for pair pruning or returning the final result, if $R$ is the root.}

\begin{rules}
\label{rule:return-simplified}
 If $\fk{R}$ exists in the head of a rule, we produce the rule
\begin{align*}
     {R}_{\mathsf{join}}(\vec{w}) & \obtainedfrom R(\vec{x}, \vec{y}), \lnot \fk{R}(\vec{x}).
\end{align*}
Otherwise, we produce the rule
\begin{align*}
     {R}_{\mathsf{join}}(\vec{w}) & \obtainedfrom R(\vec{x}, \vec{y}).
\end{align*}
\end{rules}

%
%\begin{rules}
%\label{rule:return}
%Let $R$ the argument for \textsc{ReturnPhase}. If in the previous phases the IDB  $\bk{R}(\vec{x})$ is introduced, then we produce the rule
%\begin{align}
%     \gk{R}(\vec{x}) & \obtainedfrom R(\vec{x}, \vec{y}), \lnot \bk{R}(\vec{x}).
%\end{align}
%Otherwise, we produce the rule
%\begin{align}
%     \gk{R}(\vec{x}) & \obtainedfrom R(\vec{x}, \vec{y}).
%\end{align}
%\end{rules}

\begin{example}
Figure~\ref{fig:example-rewriting} shows the three exit rules for $\examplequery$---one rule for each node in the PPJT in Figure~\ref{fig:join-tree}. We will use the boolean predicate $\jk{\relation{Employee}}$ to determine whether \texttt{True} is the consistent answer to the running query. \qed
\end{example}

\introparagraph{Runtime Analysis} It is easy to see that \textbf{Rule 1, 3, and 4} can be evaluated in linear time. We now argue how to evaluate \textbf{Rule 2} in linear time as well. Indeed, instead of performing the self-join on the key, it suffices to create a hash table using the primary key as the key (which can be constructed in linear time). Then, for every value of the key, we can easily check whether all tuples in the block have the same value at the $i$-th attribute.

%Now we present some rule-level optimizations for Rule~\ref{rule:good-join},~\ref{rule:bad-key} and~\ref{rule:return}. Rule~\ref{rule:good-join} and~\ref{rule:bad-key} can be combined into Rule~\ref{rule:bad-key-simplified}.

%\begin{figure}
%\begin{align*}
%     \fk{\relation{Employee}}(x) & \obtainedfrom \relation{Employee}(x, y, z_3), z_3 \neq y. \\
%     \fk{\relation{Employee}}(x) & \obtainedfrom \relation{Employee}(x, y, y), \lnot \relation{Mgr}_{\mathsf{join}}(y, x). \\
%     \gk{\relation{Employee}} & \obtainedfrom \relation{Employee}(x, y, y), \lnot \fk{\relation{Employee}}(x). \\
%     \fk{\relation{Mgr}}(y) & \obtainedfrom \relation{Mgr}(y, x, z_3), z_3 \neq 2020. \\
%    \fk{\relation{Mgr}}(y) & \obtainedfrom \relation{Mgr}(y, x, 2020), \relation{Mgr}(y, z_2, 2020), z_2 \neq x. \\
%     \relation{Mgr}_{\mathsf{join}}(y, x) & \obtainedfrom \relation{Mgr}(y, x, 2020), \lnot \fk{\relation{Mgr}}(y). \\
%.   \fk{\relation{Mgr}}(y) & \obtainedfrom \relation{Mgr}(y, x, 2020), \lnot \relation{Contact}_{\mathsf{join}}(y, x). \\
%     \fk{\relation{Contact}}(y) & \obtainedfrom \relation{Contact}(y, z_1), \relation{Contact}(y, x), z_1 \neq x. \\
%     \relation{Contact}_{\mathsf{join}}(y, x) & \obtainedfrom \relation{Contact}(y, x), \lnot \fk{\relation{Contact}}(y).
%\end{align*}
%\caption{The non-recursive rules for $\cqa{\examplequery}$.}
%\end{figure}

\revb{
\introparagraph{Correctness arguments}
Let $q$ be an acyclic BCQ with a PPJT $(\tau, R)$ and $\db$ an instance for $\cqa{q}$. Our rewriting \textbf{Rules 1, 2, 3, 4} are motivated to ensure their \emph{soundness}: if the predicate $R_{\mathsf{join}}$ is nonempty when our rewriting is executed on $\db$, then every consistent repair of $\db$ must satisfy $q$. It remains to argue their \emph{completeness}: if every consistent repair of $\db$ satisfies $q$, then the predicate $R_{\mathsf{join}}$ must be nonempty after executing the rules on $\db$.

The completeness of our rewriting rules is guaranteed by properties of unattacked atoms and the recursive definition of a PPJT. 
If an atom $R$ is unattacked in a BCQ $q$, Lemma 4.4 in \cite{KoutrisW17} establishes the following: 
\begin{quote}
\emph{Every consistent repair of $\db$ satisfies $q$ if and only if there is a nonempty set of tuples of $R$ that contribute to a join in all consistent repairs of $\db$.  }
\end{quote}
Our recursive construction of a PPJT $(\tau, R)$ ensures that for each rooted subtree $(\tau', S)$ of $(\tau, R)$, $S$ is unattacked in $q_{\tau'}$. 
Therefore, it suffices to compute the tuples in $S$ that could contribute to a consistent answer to $q_{\tau'}$ at each recursive step in a bottom-up fashion, eventually returning the consistent answer to $q$ in $\db$. 

The formal correctness proof is in Appendix~\ref{sec:correctness-boolean}.
}
\subsection{Correctness proof}
\label{sec:correctness-boolean}

In this section, we prove Theorem~\ref{thm:main:boolean}. 

\begin{definition}
\label{defn:good-key}
Let $\db$ be a database instance for $\cqa{q}$ and $R(\underline{\vec{x}}, \vec{y})$ an atom in $q$. We define the good keys of $R$ with respect to query $q$ and $\db$, denoted by $\goodkey{R}{q}{\db}$, as follows: 
\begin{align*}
\goodkey{R}{q}{\db} &:= \{\vec{c} \mid \db\ \text{is a ``yes''-instance for } \cqa{q_{\vec{x} \rightarrow \vec{c}}}\}.
\end{align*}
\end{definition}

Let $q$ be a self-join-free acyclic BCQ with a PPJT $(\tau, R)$. Lemma~\ref{lemma:reification} implies that in order to solve $\cqa{q}$, it suffices to check whether $\goodkey{R}{q}{\db} \neq\emptyset$. 



\begin{lemma}
\label{lemma:reification}
Let $q$ be a self-join-free acyclic BCQ with a PPJT $(\tau, R)$. Let $\db$ be a database instance for $\cqa{q}$. Then the following statements are equivalent:
\begin{enumerate}
\item $\db$ is a ``yes''-instance for $\cqa{q}$; and
\item $\goodkey{R}{q}{\db} \neq \emptyset$.
\end{enumerate}
\end{lemma}
\begin{proof}
By Lemma 4.4 in \cite{KoutrisW17}, we have that $\db$ is a ``yes''-instance for $\cqa{q}$ if and only if there exists a sequence of constant $\vec{c}$ such that $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{x} \rightarrow \vec{c}]}}$, and the latter is equivelant to $\goodkey{R}{q}{\db} \neq \emptyset$ by Definition~\ref{defn:good-key}.
\end{proof}

\begin{example}
The atom $\relation{Employee}(\underline{x}, y, z)$ is unattacked in $\examplequery$. Observe that for $\text{employee\_id} = 0022$, no matter whether we choose the tuple \relation{Employee}(0022, \text{New York}, \text{New York}) or the tuple \relation{Employee}(0022, \text{Chicago}, \text{Chicago}) in a repair, the chosen tuple will join with some corresponding tuple in the \relation{Manager} and \relation{Contact} table. The query $\examplequery_{[x \rightarrow 0022]}$ will then return \texttt{True} for all repairs of database \database{Company}, and $0022 \in \goodkey{\relation{Employee}}{\examplequery}{\textbf{Company}} \neq\emptyset$. The \textbf{Company} database is then concluded to be a ``yes''-instance for $\cqa{\examplequery}$ by Lemma~\ref{lemma:reification}. 

We remark that converse also holds: if \textbf{Company} is known to be a ``yes''-instance for $\cqa{\examplequery}$, then by Lemma~\ref{lemma:reification}, the set $\goodkey{\relation{Employee}}{\examplequery}{\textbf{Company}}$ must also be nonempty.\qed 
\end{example}


The intuition behind our algorithm for computing $\goodkey{R}{q}{\db}$ is as follows. Recall that $(\tau, R)$ is a PPJT of $q$ and thus $R$ is unattacked in $q$. Let $(\tau', S)$ be any child rooted subtrees of $R$ in $(\tau, R)$. Since $(\tau, R)$ is a PPJT of $q$, then $(\tau', S)$ is also a PPJT of the subquery $q_{\tau'}$ of $q$. By Lemma~\ref{lemma:reification}, the set $\goodkey{S}{q_{\tau'}}{\db}$ encodes the answer for $\cqa{q_{\tau'}}$. To compute $\goodkey{R}{q}{\db}$, since $R$ and $S$ are adjacent in the join tree $\tau$ of $q$, we will use the set $\goodkey{S}{q_{\tau'}}{\db}$ that we have recursively computed to ``prune'' the primary keys of $R$. The term ``pair-pruning'' is motivated by this process of pruning the primary keys by considering one pair of atoms at a time. Lemma~\ref{lemma:pair-pruning} formalizes this idea and is proved in Appendix~\ref{sec:missing-proofs} of the extended version of this paper.

\begin{lemma}
\label{lemma:pair-pruning}
     Let $R(\underline{\vec{x}}, \vec{y})$ be an atom in an acyclic self-join-free BCQ~$q$ with a PPJT $(\tau, R)$. Let $\db$ be an instance for $\cqa{q}$. For every sequence $\vec{c}$ of constants, of the same length as $\vec{x}$, the following are equivalent:
     \begin{enumerate}
          \item $\vec{c} \in \goodkey{R}{q}{\db}$; and \label{it:whole}
          \item 
          \label{it:pair-algo}
the block $R(\underline{\vec{c}},*)$ of $\db$ is non-empty and for every fact $R(\underline{\vec{c}},\vec{d})$ in $\db$, the following hold:
          \begin{enumerate}
          \item $\{R(\underline{\vec{c}},d)\}$ satisfies the BCQ $()\obtainedfrom R(\underline{\vec{x}}, \vec{y})$; and
          \label{it:self-pruning}
          \item 
          \label{it:pair-pruning}
for every child subtree $(\tau_S, S)$ of $(\tau, R)$, there exists  $\vec{s} \in \goodkey{S}{q_{\tau_S}}{\db}$ such that (i) all facts $S(\underline{\vec{s}}, \vec{t})$ agree on the joining variables in $\var{R} \cap \var{S}$ and (ii) for every fact $S(\underline{\vec{s}}, \vec{t})$ in $\db$, the pair $\{R(\underline{\vec{c}}, \vec{d})$, $S(\underline{\vec{s}}, \vec{t})\}$ satisfies the BCQ 
$()\obtainedfrom R(\underline{\vec{x}}, \vec{y}), S(\underline{\vec{u}}, \vec{v}),$ 
where $S(\underline{\vec{u}}, \vec{v})$ is the $S$-atom of $q$.
          \end{enumerate}
          
     \end{enumerate}   
\end{lemma}


\begin{proof}[Proof of Theorem~\ref{thm:main:boolean}]
It suffices to present rewriting rules to compute each $\goodkey{R}{q}{\db}$ for each atom $R$ in $q$ by Lemma~\ref{lemma:pair-pruning} , and show that these rewriting rules are equivalent to those presented in Section~\ref{sec:datalog}, which are shown to run in linear time. We denote $R_{\mathsf{gk}}$ as the Datalog predicate for $\goodkey{R}{q}{\db}$. 
It is easy to see that \textbf{Rule 1} computes all blocks of $R$ violating item~\ref{it:self-pruning} of Lemma~\ref{lemma:pair-pruning}. 

To compute the blocks of $R$ violating item~\ref{it:pair-pruning}, we denote $R_{\mathsf{gki}}$ as the predicate for the subset of $R_{\mathsf{gk}}$ that satisfies condition (i) of item~\ref{it:pair-pruning}.
For each child $S(\underline{\vec{u}}, \vec{v})$ of $R$ in a PPJT, let $\vec{w}$ be a sequence of all variables in $\var{R} \cap \var{S}$. The following rules find all blocks in $R$ that violate condition (ii) of item~\ref{it:pair-pruning}.
\begin{align}
\label{rule:join}
S_{\mathsf{join}}(\vec{w}) & \obtainedfrom S(\underline{\vec{u}}, \vec{v}), S_{\mathsf{gki}}(\vec{u}). \\ 
\label{rule:pp}
\fk{R}(\vec{x}) & \obtainedfrom R(\vec{x}, \vec{y}) \lnot S_{\mathsf{join}}(\vec{w}).
\end{align}
We then compute the predicate $R_{\mathsf{gk}}$ denoting $\goodkey{R}{q}{\db}$ with
\begin{align}
\label{rule:gk}
R_{\mathsf{gk}}(\vec{x}) &\obtainedfrom R(\underline{x}, \vec{y}), \lnot \fk{R}(\vec{x}).
\end{align}
If $R$ has a parent, then we may compute all blocks in $R$ violating condition (i) of item~\ref{it:pair-pruning} using the following rules for every variable at the $i$-th position of $\vec{y}$,
\begin{align}
\label{rule:gkinot}
R_{\mathsf{gk}^{\lnot}}(\vec{x}) &\obtainedfrom R(\vec{x}, \vec{y}), R(\vec{x}, \vec{y}'), y_i \neq y_i'. \\ 
\label{rule:gki}
R_{\mathsf{gki}}(\vec{x}) & \obtainedfrom R_{\mathsf{gk}}(\vec{x}), \lnot R_{\mathsf{gk}^{\lnot}}(\vec{x}). 
\end{align}
% For $R$, the root of the PPJT $(\tau, R)$ of $q$, \textbf{Rule 1} is the only self-pruning rule, computing exactly the blocks $R(\underline{\vec{c}}, *)$ that violates item~\ref{it:self-pruning}. 
% For each child rooted subtree $(\tau', S)$, \textbf{Rule 3} computes exactly the blocks $R(\underline{\vec{c}}, *)$ that violates item~\ref{it:pair-pruning}. Therefore \textbf{Rule 1, 3} together compute the blocks $R(\underline{\vec{c}}, *)$ that violates either item~\ref{it:self-pruning} or item~\ref{it:pair-pruning}. Finally, \textbf{Rule 4} computes the Boolean predicate $R_{\mathsf{join}}$, denoting whether there is a block $R(\underline{\vec{c}}, *)$ that satisfies both item~\ref{it:self-pruning} and~\ref{it:pair-pruning}. Hence the Boolean predicate $R_{\mathsf{join}}$ is nonempty if and only if $\goodkey{R}{q}{\db} \neq \emptyset$.

% For any rooted subtree $(\tau', S)$ of $(\tau, R)$, let $T$ be the parent of $S(\underline{\vec{x'}}, \vec{y'})$ in $(\tau, R)$ and let $\vec{w}$ be a sequence of joining variables between $S$ and $T$. \textbf{Rule 1, 3} still correctly compute the block $S(\underline{\vec{s}}, *)$ that violates either item~\ref{it:self-pruning} or~\ref{it:pair-pruning}. Note that if there are two facts $f_1 = S(\underline{\vec{s}}, \vec{t_1})$ and $f_2 = S(\underline{\vec{s}}, \vec{t_2})$ that do not agree on some variable $z$ in $\var{\vec{y'}} \cap \var{T}$, then any fact $T(\underline{\vec{c}}, \vec{d})$ cannot join with both $S(\underline{\vec{s}}, \vec{t_1})$ and $S(\underline{\vec{s}}, \vec{t_2})$ at the same time, or otherwise $f_1$ and $f_2$ would have to agree on the variable $z$, a contradiction. Hence we may further remove blocks $S(\underline{\vec{s}}, *)$ that contain two facts disagreeing on any joining variable $z \in \var{\vec{y'}} \cap \var{T}$, which is achieved by \textbf{Rule 2}. Consequently, for every block $S(\underline{\vec{s}}, *)$ where $\vec{s}$ is not included in $S_{\mathsf{fkey}}$ due to \textbf{Rule 1, 2, 3}, all facts in blocks $S(\underline{\vec{s}}, *)$ agree on the variables $\vec{w}$, a sequence of joining variables between $S$ and $T$, which is computed by \textbf{Rule 4}.
Now we explain why Rules~(\ref{rule:join}) through~(\ref{rule:gki}) are equivalent to \textbf{Rule 2, 3, 4}.
First, the head $R_{\mathsf{gk}^{\lnot}}$ of Rule~(\ref{rule:gkinot}) can be safely renamed to $\fk{R}$ and yield \textbf{Rule 2}. Rule~(\ref{rule:pp}) is equivalent to \textbf{Rule 3}. Finally, Rules~(\ref{rule:join}),~(\ref{rule:gk}) and~(\ref{rule:gki}) can be merged to \textbf{Rule 4} since to compute each $S_{\mathsf{join}}$, we only need $S(\vec{u}, \vec{v})$ and $\fk{S}$. Note that the Rule~(\ref{rule:join}) for the atom $R$ will have $0$ arity if $R$ is the root of the PPJT. 
\end{proof}

% The complete proof of Theorem~\ref{thm:main:boolean} is in Appendix~\ref{sec:missing-proofs} of the extended version of this paper. \xiating{Is this proof formal enough? Do we need to make it more sketchy and put a formal inductive version in the appendix?}


% \jef{I slightly reformulated the following lemma and placed it in front of the definition of PPJT.
% If that is okay, then the lemma can be omitted here.}
% \begin{lemma}[\cite{KoutrisW17}]
% \label{lemma:reification}
% Let $q$ be a self-join-free BCQ whose attack graph is acyclic and $R(\underline{\vec{x}}, \vec{y})$ an unattacked atom in $q$. Let $\db$ be an instance for $\cqa{q}$. Then the following statements are equivalent:
% \begin{enumerate}
%      \item $\db$ is a ``yes''-instance for $\cqa{q}$; and
%      \item $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{x} \rightarrow \vec{c}]}}$ for some sequence of constants $\vec{c}$.
% \end{enumerate} 
% \end{lemma}

% If $R(\underline{\vec{x}}, \vec{y})$ is an atom of a query $q$ with a PPJT  $(\tau, R)$, then $R$ is not attacked in $q$ by definition. By Lemma~\ref{lemma:reification}, it suffices to compute \emph{all} keys $\vec{c}$ in the relation $R$ such that $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{x} \rightarrow \vec{c}]}}$, called the \emph{good keys} of $R$ with respect to the query $q$ and the database $\db$.



%The term ``pair-pruning'' is motivated by item~\ref{it:pair-pruning}.
%To check if $()\obtainedfrom R(\underline{\vec{x}}, \vec{y}), S(\underline{\vec{x}'}, \vec{y}')$ holds, one can use that the tuple $S(\underline{\vec{s}}, \vec{t})$ already satisfies 
% $()\obtainedfrom S(\underline{\vec{x}'}, \vec{y}')$.
%Therefore, it suffices to check if $R(\underline{\vec{c}}, \vec{d})$ and $S(\underline{\vec{s}}, \vec{t})$ agree on the variables shared by  $R(\underline{\vec{x}}, \vec{y})$ and $S(\underline{\vec{x}'},\vec{y'})$.    

%Lemma~\ref{lemma:pair-pruning} immediately implies that if $q$ has a PPJT $(\tau, R)$, the set $\goodkey{R}{q}{\db}$ can be recursively computed by items~\ref{it:self-pruning} and~\ref{it:pair-pruning}, which can be na\"ively implemented in $O(N^2)$ time. 


\subsection{Extension to Non-Boolean Queries}
\label{sec:nonboolean}

Let $q(\vec{u})$ be an acyclic self-join-free CQ with free variables $\vec{u}$, and $\db$ be a database instance. If $\vec{c}$ is a sequence of constants of the same length as $\vec{u}$, we say that $\vec{c}$ is a {\em consistent answer} to $q$ on $\db$ if $\vec{c} \in q(I)$ in every repair $I$ of $\db$.
Furthermore, we say that $\vec{c}$ is a {\em possible answer} to $q$ on $\db$ if $\vec{c} \in q(\db)$. It can be easily seen that for CQs every consistent answer is a possible answer.


 Lemma~\ref{lemma:parameterization} reduces computing the consistent answers of non-Boolean queries to that of Boolean queries.
% suggests that the free variables of $q$ can be treated as constants. 


\begin{lemma}
\label{lemma:parameterization}
Let $q$ be a CQ with free variables $\vec{u}$, and let $\vec{c}$ be a sequence of constants of the same length as $\vec{u}$. Let $\db$ be an database instance. Then $\vec{c}$ is a consistent answer to $q$ on $\db$ 
if and only if $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$. 
\end{lemma}

 If $q$ has free variables $\vec{u} = (u_1, u_2, \dots, u_n)$, we say that $q$ admits a PPJT if the Boolean query $q_{[\vec{u} \rightarrow \vec{c}]}$ admits a PPJT, where $\vec{c} = (c_1, c_2, \dots, c_n)$ is a sequence of distinct constants.
 We can now state our main result for non-Boolean CQs.


\begin{theorem}\label{thm:main:full}
Let $q$ be an acyclic self-join-free Conjunctive Query that admits a PPJT, and $\db$ be a database instance of size $N$.
Let $\mathsf{OUT}_p$ be the set of possible answers to $q$ on $\db$,
and $\mathsf{OUT}_c$ the set of consistent answers to $q$ on $\db$. Then:
\begin{packed_enum}
\item The set of consistent answers can be computed in time $O(N \cdot |\mathsf{OUT}_p|)$; and
\item Moreover, if $q$ is full, the set of consistent answers can be computed in time $O(N + |\mathsf{OUT}_c|)$.
\end{packed_enum}
\end{theorem}

To contrast this with Yannakakis result, for acyclic full CQs we have a running time of $O(N + |\mathsf{OUT}|)$, and a running time of $O(N \cdot |\mathsf{OUT}|)$ for general CQs. 

%
%\begin{theorem}[\cite{DBLP:conf/vldb/Yannakakis81}]
%\label{thm:yannakakis}
%Let $q$ be an acyclic self-join-free Conjunctive Query, and $\db$ a database instance of size $N$. Let $\mathsf{OUT} = q(\db)$. Then:
%\begin{packed_enum}
%\item There exists an algorithm that evaluates ${q}$ on $\db$  in time $O(N \cdot |\mathsf{OUT}|)$.
%\item If $q$ is boolean, there exists an algorithm  that evaluates ${q}$ on $\db$ in time $O(N)$.
%\item If $q$ is full, there exists an algorithm  that evaluates ${q}$ on $\db$ in time $O(N + |\mathsf{OUT}|)$.
%\end{packed_enum}
%\end{theorem}

\begin{proof}
% By Lemma~\ref{lemma:parameterization}, we can first compute $q(\db)$ to obtain a set of {\em possible} answers, which must contain all the consistent answers of $q$ on $\db$. We then return all answers $\vec{c} \in q(\db)$ such that $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$. This approach gives an algorithm with running time $O(N \cdot |\mathsf{OUT}_p|)$.

% If $q$ is full, there is an algorithm that computes the set of consistent answers even faster. The algorithm proceeds by first computing the consistent part $R^c$ for any relation $R$, that is, the set of facts that do not conflict with any other fact in $R$. Next, it evaluates $q$ on just the consistent part of the database. The algorithm is correct, since by Lemma~\ref{lemma:parameterization}, all constants $\vec{c}$ such that the block $R(\vec{c}, *)$ is inconsistent would be pruned, and thus $R^c$ is precisely the relation obtained by filtering the keys of $R$ on $\gk{R}$.
\reva{Our algorithm first evaluates $q$ on $\db$ to yield a set $S$ of size $|\mathsf{OUT}_{p}|$ in time $O(N \cdot |\mathsf{OUT}_p|)$.  
Here the set $S$ must contain all the consistent answers of $q$ on $\db$. By Lemma~\ref{lemma:parameterization}, we then return all answers $\vec{c} \in S$ such that $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$, which runs in $O(N)$ by Theorem~\ref{thm:main:boolean}. This approach gives an algorithm with running time $O(N \cdot |\mathsf{OUT}_p|)$.

If $q$ is full, there is an algorithm that computes the set of consistent answers even faster. The algorithm proceeds by (i) removing all blocks with at least two tuples from $\db$ to yield $\db^c$ and (ii) evaluating $q$ on $\db^c$. 
It suffices to show that every consistent answer to $q$ on $\db$ is an answer to $q$ on $\db^c$. 
Assume that $\vec{c}$ is a consistent answer to $q$ on $\db$. Consider $q_{[\vec{u} \rightarrow \vec{c}]}$, a disconnected CQ where $\vec{u}$ is a sequence of all variables in $q$. Its \FO-rewriting effectively contains \textbf{Rule 1} for each atom in $q_{[\vec{u} \rightarrow \vec{c}]}$, which is equivalent to step (i), and then checks whether $\db^c$ satisfies $q_{[\vec{u} \rightarrow \vec{c}]}$ by Lemma~B.1 of~\cite{DBLP:conf/pods/KoutrisOW21}. By Lemma~\ref{lemma:parameterization}, $\db$ is a ``yes''-instance for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$, and thus the \FO-rewriting concludes that $\db^c$ satisfies $q_{[\vec{u} \rightarrow \vec{c}]}$, i.e.\ $\vec{c}$ is an answer to $q$ on $\db^c$.
In our algorithm, step (i) runs in $O(N)$ and since $q$ is full, step (ii) runs in time $O(N + |\mathsf{OUT}_c|)$.
}
\end{proof}

% Let $\vec{c} = (c_1, c_2, \dots, c_n) \in U$. If $q_{[\vec{u} \rightarrow \vec{c}]}$ has a PPJT, then there is a non-recursive datalog program $P_{\vec{c}}$ that solves $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$. For a different answer $\vec{c'} = (c_1', c_2', \dots, c_n')$, the non-recursive datalog program $P_{\vec{c'}}$ for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$ can be obtained by replacing each constant $c_i$ in $P_{\vec{c}}$ with $c_i'$. 

\introparagraph{Rewriting for non-Boolean Queries}
Let $\vec{c} = (c_1, c_2, \dots, c_n)$ be any sequence of distinct constants that do not appear in~$q$. If $q_{[\vec{u} \rightarrow \vec{c}]}$ has a PPJT, the Datalog rewriting for $\cqa{q}$ can be obtained as follows:
%
\begin{packed_enum}
\item Produce the program $P$ for $\cqa{q_{[\vec{u} \rightarrow \vec{c}]}}$ using the rewriting algorithm for Boolean queries (Subsection~\ref{sec:datalog}).
\item Replace each occurrence of the constant $c_i$ in $P$ with the free variable $u_i$.
\item Add the rule: $\mathsf{ground}(\vec{u}) \obtainedfrom \mathsf{body}(q)$.
\item For a relation $T$, let $\vec{u}_T$ be a sequence of all free variables that occur in the subtree rooted at $T$. Then, append $\vec{u}_T$ to every occurrence of $\jk{T}$ and $\fk{T}$.
\item For any rule of $P$ that has a free variable $u_i$ that is unsafe, add the atom $\mathsf{ground}(\vec{u})$ to the rule.
\end{packed_enum}

\begin{example}
Consider the non-Boolean query 
%
$$\examplequerynb(w) \obtainedfrom \mathsf{Employee}(\underline{x}, y, z), \mathsf{Manager}(\underline{y}, x, w), \mathsf{Contact}(\underline{y}, x).$$ 

Note that the constant \texttt{2020} in $\examplequery$ is replaced by the free variable $w$ in $\examplequerynb$. Hence, the program $P$ for $\cqa{\examplequerynb_{[w \rightarrow c]}}$ is the same as Figure~\ref{fig:example-rewriting}, with the only difference that \texttt{2020} is replaced by the constant $c$.
The ground rule produced is:
%
$$\mathsf{ground}(w) \obtainedfrom \mathsf{Employee}({x}, y, z), \mathsf{Manager}({y}, x, w), \mathsf{Contact}({y}, x).$$ 

To see how the rule of $P$ would change for the non-Boolean case, consider the self-pruning rule for $\mathsf{Contact}$. This rule would remain as is, because it contains no free variable and the predicate $\fk{\relation{Contact}}$ remains unchanged. In contrast, consider the first self-pruning rule for $\mathsf{Manager}$, which in $P$ would be:
%
$$ \fk{\relation{Manager}}(y_1)  \obtainedfrom \relation{Manager}(y_1, y_2, y_3), y_3 \neq w. $$

Here, $w$ is unsafe, so we need to add the atom $\mathsf{ground}(w)$. Additionally, $w$ is now a free variable in the subtree rooted at $\relation{Manager}$, so the predicate $\fk{\relation{Manager}}(y_1)$ becomes $\fk{\relation{Manager}}(y_1,w) $. The transformed rule will be:
%
$$ \fk{\relation{Manager}}(y_1,w)  \obtainedfrom \relation{Manager}(y_1, y_2, y_3), y_3 \neq w, \mathsf{ground}(w).$$
%
The full rewriting for $\examplequerynb$ can be seen in Figure~\ref{fig:example-nonboolean}. \qed
\end{example}

The above rewriting process may introduce cartesian products in the rules. In the next section, we will see how we can tweak the rules in order to avoid this inefficiency.


\begin{figure*}[t]
\small
\subfloat[Yannakakis' Algorithm]{
     \begin{tikzpicture}[level distance=10em,
     every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
     brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
     \tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=5mm, rectangle, rounded corners}};

     \node (E-exit) [draw=none] {$\relation{Employee}_{\mathsf{join}}(w) \obtainedfrom \relation{Employee}(x, y, z), \relation{Manager}_{\mathsf{join}}(y, x, w).$};

     \node (M-exit) [below = 2.1 cm of E-exit.west, anchor=west, draw=none]{       
           $\relation{Manager}_{\mathsf{join}}(y, x,w)  \obtainedfrom \relation{Manager}(y, x, w), \relation{Contact}_{\mathsf{join}}(y, x).$}; 
     
     \node (C-exit) [below =2.15 cm of M-exit.west, anchor=west, draw=none] {
          $\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x).$};
     

     \path[->] (E-exit.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
     {} ($(3,0.2)+(M-exit.north west)$) ;

     \path[->] (M-exit.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
     {} ($(C-exit.north west)+(3,0.2)$) ;

     \node (box1) [draw=blue, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (E-exit)] {};
     
      \node (box2) [draw=red, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (M-exit)] {};    

     \node (box3) [draw=brown, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (C-exit)] {};
     \node [below=0.4cm of box3, white] {};
     \end{tikzpicture}     

}
\quad
\subfloat[PPJT extended to non-Boolean queries]{
     \begin{tikzpicture}[level distance=10em,
     every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
     brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
     \tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=5mm, rectangle, rounded corners}};

     \node (ground) [draw=none] {
          $\mathsf{ground}(w) \obtainedfrom \mathsf{Employee}({x}, y, z), \mathsf{Manager}({y}, x, w), \mathsf{Contact}({y}, x).$};
     % \draw [brace]  (ground.south west) -- (ground.north west) node[midway, left=15pt, black,draw=none]{\textsc{Ground-Rule}};    

     \node (E-exit) [below = 1cm of ground.west, anchor=west, draw=none] {
          \textbf{R4: }$\relation{Employee}_{\mathsf{join}}(w) \obtainedfrom \relation{Employee}(x, y, z), \lnot \fk{\relation{Employee}}(x,w), \mathsf{ground}(w).$};
     % \draw [brace]  (E-exit.south west) -- (E-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};  

     \node (E-self) [below = 0.6cm of E-exit.west, anchor=west, draw=none] {   
          \textbf{R3: }$\fk{\relation{Employee}}(x,w)  \obtainedfrom \relation{Employee}(x, y, z), \lnot \relation{Manager}_{\mathsf{join}}(y, x,w), \mathsf{ground}(w).$};
     % \draw [brace]  (E-self.south west) -- (E-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

     \node (M-exit) [below = 1.5 cm of E-self.west, anchor=west, draw=none]{       
           \textbf{R4: }$\relation{Manager}_{\mathsf{join}}(y, x,w)  \obtainedfrom \relation{Manager}(y, x, w), \lnot \fk{\relation{Manager}}(y), \mathsf{ground}(w).$}; 
     % \draw [brace]  (M-exit.south west) -- (M-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};  
           
     \node (M-self) [below =0.9cm of M-exit.west, anchor=west, draw=none]{ 
           $\begin{aligned}
     \textbf{R1: }&\fk{\relation{Manager}}(z_1, w)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq w, \mathsf{ground}(w). \\
     \textbf{R2: }&\fk{\relation{Manager}}(y, w)  \obtainedfrom \relation{Manager}(y, x, w), \relation{Manager}(y, z_1, w), z_1 \neq x. \\
     \textbf{R3: }& \fk{\relation{Manager}}(y, w)  \obtainedfrom \relation{Manager}(y, x, w), \lnot \relation{Contact}_{\mathsf{join}}(y, x), \mathsf{ground}(w).
     \end{aligned}$};
     % \draw [brace]  (M-self.south west) -- (M-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

     \node (C-exit) [below =1.9 cm of M-self.west, anchor=west, draw=none] {
          \textbf{R4: }$\relation{Contact}_{\mathsf{join}}(y, x)  \obtainedfrom \relation{Contact}(y, x), \lnot \fk{\relation{Contact}}(y).$};
     % \draw [brace]  (C-exit.south west) -- (C-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};

     \node (C-self) [below = 0.6cm of C-exit.west, anchor = west, draw=none] {
          \textbf{R2: }$\fk{\relation{Contact}}(y)  \obtainedfrom \relation{Contact}(y, x), \relation{Contact}(y, z_1), z_1 \neq x.$};
     % \draw [brace]  (C-self.south west) -- (C-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};


     \path[->] (E-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
     {} ($(3,0.2)+(M-exit.north west)$) ;

     % \draw [brace]   (PP.north east) -- (PP.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

     \path[->] (M-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
     {} ($(C-exit.north west)+(3,0.2)$) ;

     % \draw [brace]   (PP2.north east) -- (PP2.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

     \node (box1) [draw=blue, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (E-exit) (E-self)] {};
     
      \node (box2) [draw=red, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (M-exit) (M-self)] {};    

     \node (box3) [draw=brown, line width=1pt,
                                    dash pattern=on 1pt off 4pt on 6pt off 4pt,
                                     inner sep=1mm, rectangle, rounded corners,  fit = (C-exit) (C-self)] {};                                      
% \node [right = 13mm of box1, draw=none, above] {{\color{blue} $\relation{Employee}(\underline{x},z,z)$}}; 
% \node [right = 15mm of box2, draw=none, above] {{\color{red} $\relation{Manager}(\underline{z},x,w)$}}; 
% \node [right = 10mm of box3, draw=none, above] {{\color{brown} $\relation{Contact}(\underline{z},x)$}}; 
                                                        
     \end{tikzpicture}    
     \label{fig:example-nonboolean}
}
\caption{The non-recursive Datalog program for $\examplequerynb$ and $\cqa{\examplequerynb}$.}

\end{figure*}

% \begin{figure*}[t]
% \begin{tikzpicture}[level distance=10em,
% every node/.style = {line width=0.5pt, shape=rectangle, text centered, anchor=center, rounded corners, draw, align=center}, grow=right,
% brace/.style = {black,decorate, decoration = {brace, raise=10pt,amplitude=3pt}}]
% \tikzset{blue dotted/.style={draw=blue!50!white, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=5mm, rectangle, rounded corners}};

% \node (ground) [draw=none] {
% 	$\mathsf{ground}(w) :- \mathsf{Employee}({x}, z, z), \mathsf{Manager}({z}, x, w), \mathsf{Contact}({z}, x).$};
% \draw [brace]  (ground.south west) -- (ground.north west) node[midway, left=15pt, black,draw=none]{\textsc{Ground-Rule}};	

% \node (E-exit) [below = 1cm of ground.west, anchor=west, draw=none] {
% 	$\relation{Employee}_{\mathsf{join}}(w) \obtainedfrom \relation{Employee}(x, y, y), \lnot \fk{\relation{Employee}}(x,w), \mathsf{ground}(w).$};
% \draw [brace]  (E-exit.south west) -- (E-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};	 

% \node (E-self) [below = 0.75cm of E-exit.west, anchor=west, draw=none] {	
% 	$\fk{\relation{Employee}}(z_1,w)  \obtainedfrom \relation{Employee}(z_1, z_2, z_3), z_3 \neq z_2, \mathsf{ground}(w). $};
% \draw [brace]  (E-self.south west) -- (E-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

% \node (M-exit) [below = 2 cm of E-self.west, anchor=west, draw=none]{ 	 
% 	 $\relation{Manager}_{\mathsf{join}}(z, x,w)  \obtainedfrom \relation{Manager}(z, x, w), \lnot \fk{\relation{Manager}}(z).$}; 
% \draw [brace]  (M-exit.south west) -- (M-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};	 
	 
% \node (M-self) [below =1cm of M-exit.west, anchor=west, draw=none]{ 
% 	 $\begin{aligned}
% 	 &\fk{\relation{Manager}}(z_1,w)  \obtainedfrom \relation{Manager}(z_1, z_2, z_3), z_3 \neq w, \mathsf{ground}(w).  \\
% 	 & \fk{\relation{Manager}}(z,w)   \obtainedfrom \relation{Manager}(z, x, w), \relation{Manager}(z, z_1, z_2), z_1 \neq x.
% 	 \end{aligned}$};
% \draw [brace]  (M-self.south west) -- (M-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};

% \node (C-exit) [below =2 cm of M-self.west, anchor=west, draw=none] {
% 	$\relation{Contact}_{\mathsf{join}}(z, x)  \obtainedfrom \relation{Contact}(z, x), \lnot \fk{\relation{Contact}}(z).$};
% \draw [brace]  (C-exit.south west) -- (C-exit.north west) node[midway, left=15pt, black,draw=none]{\textsc{Exit-Rule}};

% \node (C-self) [below = 0.75cm of C-exit.west, anchor = west, draw=none] {
% 	$\fk{\relation{Contact}}(z)  \obtainedfrom \relation{Contact}(z, x), \relation{Contact}(z, z_1), z_1 \neq x.$};
% \draw [brace]  (C-self.south west) -- (C-self.north west) node[midway, left=15pt, black,draw=none]{\textsc{Self-Pruning}};


% \path[->] (E-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP) [draw=none,anchor=west] 
% {$\fk{\relation{Employee}}(x,w)  \obtainedfrom \relation{Employee}(x, z, z), \lnot \relation{Manager}_{\mathsf{join}}(z, x,w), \mathsf{ground}(w).$} ($(3,0.2)+(M-exit.north west)$) ;

% \draw [brace]   (PP.north east) -- (PP.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

% \path[->] (M-self.south west)+(3,-0.2) edge [line width=0.8pt] node (PP2) [draw=none,anchor=west] 
% {$ \fk{\relation{Manager}}(z,w)  \obtainedfrom \relation{Manager}(z, x, w), \lnot \relation{Contact}_{\mathsf{join}}(z, x). $} ($(C-exit.north west)+(3,0.2)$) ;

% \draw [brace]   (PP2.north east) -- (PP2.south east) node[midway, right=15pt, black,draw=none]{\textsc{Pair-Pruning}};

% \node (box1) [draw=blue, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (E-exit) (E-self)] {};
% \node [right = 13mm of box1, draw=none, above] {{\color{blue} $\relation{Employee}(\underline{x},z,z)$}}; 

%  \node (box2) [draw=red, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (M-exit) (M-self)] {};    
% \node [right = 15mm of box2, draw=none, above] {{\color{red} $\relation{Manager}(\underline{z},x,w)$}}; 

% \node (box3) [draw=brown, line width=1pt,
%                                dash pattern=on 1pt off 4pt on 6pt off 4pt,
%                                 inner sep=1mm, rectangle, rounded corners,  fit = (C-exit) (C-self)] {};                                      
% \node [right = 10mm of box3, draw=none, above] {{\color{brown} $\relation{Contact}(\underline{z},x)$}}; 
                                                        
% \end{tikzpicture}
% \caption{The non-recursive Datalog program produced for $\cqa{\examplequerynb}$.}
% \label{fig:example-nonboolean}
% \end{figure*}



